Succinctness of Cosafety Fragments of LTL via Combinatorial Proof Systems (extended version)

This paper focuses on succinctness results for fragments of Linear Temporal Logic with Past (LTL) devoid of binary temporal operators like until, and provides methods to establish them. We prove that there is a family of cosafety languages (Ln)_{n>=1} such that Ln can be expressed with a pure future formula of size O(n), but it requires formulae of size 2^{\Omega}(n) to be captured with past formulae. As a by-product, such a succinctness result shows the optimality of the pastification algorithm proposed in [Artale et al., KR, 2023]. We show that, in the considered case, succinctness cannot be proven by relying on the classical automata-based method introduced in [Markey, Bull. EATCS, 2003]. In place of this method, we devise and apply a combinatorial proof system whose deduction trees represent LTL formulae. The system can be seen as a proof-centric (one-player) view on the games used by Adler and Immerman to study the succinctness of CTL.

==> sections/conclusion.tex <==
%! root=../main.tex

\section{Conclusion and Future Works}
\label{sec:conclusion}

\am{below things to add to the conclusion}

\begin{itemize}
  \item summary of the paper
  \item Future work: adding until to improve the lower bound of pastification for full cosafety LTL. Show rule for until. 
  \item Future work: connections with learning
\end{itemize}


==> sections/games.tex <==

\section{Proof system}

We fix a finite alphabet $\Sigma$. A \emph{trace} $\sigma$ over $\Sigma$ is a \emph{finite, nonempty
sequence} in $\Sigma^+$.  Given $\sigma
= \seq{\sigma_0,\sigma_1,\dots,\sigma_n}$, we define the \emph{length} of
$\sigma$, denoted as $|\sigma|$, as $n+1$.

Below, let $A,B$ be sets of pairs $\pair{\sigma,i}$ such that $\sigma \in
\Sigma^+$ and $0\le i < |\sigma|$.
Given a formula $\Phi$, we write $A \models \Phi$ whenever $a \models \Phi$
for every $a \in A$, and we write $A \pperp \Phi$ whenever $a \not\models
\Phi$ for every $a \in A$.

We define $A^{\ltl{X}} \coloneqq \set{(\sigma,i+1) : (\sigma,i) \in A,\,
i < |\sigma| }$.

We say that a map $f : A \to \N$ is a \emph{future point} for $A$ whenever
$i \leq f(\sigma,i) < |\sigma|$ for every $(\sigma,i) \in A$. 
%
Given a future point $f$ of $A$, we define $f(A) \coloneqq \set{(\sigma,j)
\suchthat (\sigma,i) \in A, f(\sigma,i) = j}$.
%
We write $\FP_A$ for the set of all future points of $A$, that is $\set{
  f : A \to \N \suchthat f \text{ is a future point of } A}$.  Finally, we
define $A^{\ltl{F}} \coloneqq \bigcup_{f \in \FP_A} f(A)$.
%
All the above definitions hold for the set $B$ as well.

Here below we write the rules of the proof system for \LTLxf.

\begin{mathpar} 
  \inferrule[\ruleAtomic ($\alpha = p$ or $\alpha = \lnot p$, with
  $p\in\Sigma$)]{A \models \alpha \and B \pperp \alpha}{(A,B)}
  \and
  \inferrule[\ruleOr]{(A_1,B) \qquad (A_2,B)}{(A_1 \uplus A_2, B)}
  \and 
  \inferrule[\ruleAnd]{(A,B_1) \qquad (A,B_2)}{(A, B_1
  \uplus B_2)}\\
  \inferrule[\ruleNext]{(A^{\ltl{X}},B^{\ltl{X}}) \and |A^{\ltl{X}}| = |A|}{(A,B)}
  \and 
  \inferrule[\ruleFuture]{(f(A),B^{\ltl{F}}) \and f \in \FP_A}{(A,B)}
\end{mathpar}
Note: the \ruleFuture rule is selecting a future point for
$A$ and considering all future points for $B$.

\begin{theorem}
  The pair $(A,B)$ has a derivation tree of size $k$ if and
  only if there is a formula~$\Phi$ of cosafety LTL(X,F) of
  size $k$ such that $A \models \Phi$ and $B \pperp \Phi$.
\end{theorem}

Note: we postulate the size of a literal to be $1$,
regardless of whether it is negated or not.

\begin{proof}
  We remark that the proof is constructive, i.e., from a
  derivation tree it is possible to construct a formula, and
  vice versa.

  ($\Rightarrow$): By induction on $k$ and by cases on the
  derivation tree. 
  \begin{description}
    \item[base case: $k = 1$.] In this case the derivation
    tree is a simple instantiation of the \ruleAtomic axiom,
    and the proof is straightforward. 
    \item[induction step: $k \geq 2$.] We divide the proof
    by cases depending on the rule used at the root of the
    derivation tree. 
    \begin{description}
      \item[rule \ruleOr.] By induction hypothesis, there
      are formulae $\Phi_1$ and $\Phi_2$ such that $A_1
      \models \Phi_1$ and $A_2 \models \Phi_2$, where $A_1$
      and $A_2$ are the sets used in the \ruleOr rule, with
      $A = A_1 \uplus A_2$. Moreover, $B \pperp \Phi_1$ and
      $B \pperp \Phi_2$. Therefore, $A \models \Phi_1 \lor
      \Phi_2$ and $B \pperp (\Phi_1 \lor \Phi_2)$.
      \item[rule \ruleAnd.] By induction hypothesis, there
      are formulae $\Phi_1$ and $\Phi_2$ such that $B_1
      \pperp \Phi_1$ and $B_2 \pperp \Phi_2$, where $B_1$
      and $B_2$ are the sets used in the \ruleAnd rule, with
      $B = B_1 \uplus B_2$. Moreover, $A \models \Phi_1$ and
      $A \models \Phi_2$. Therefore, $A \models \Phi_1 \land
      \Phi_2$ and $B \pperp (\Phi_1 \land \Phi_2)$.
      \item[rule \ruleNext.] By induction hypothesis, there
      is a formula $\Phi$ such that $A^X \models \Phi$ and
      $B^X \pperp \Phi$. Notice that $|A^X| = |A|$, and so
      by definition of $A^X$, for every $(w,i) \in A$ we
      have $i < |w|$. Since moreover $(w,i+1) \models \Phi$,
      we get $A \models X \Phi$. Let us now show that $B
      \pperp X \Phi$. \emph{Ad absurdum}, suppose there is
      $(u,j) \in B$ such that $(u,j) \models X \Phi$. Then
      $j < |w|$ and $(u,j+1) \models \Phi$. This is
      contradictory, as $(u,j+1) \in B^X$ and $B^X \pperp
      \Phi$. Hence, $B \pperp X \Phi$.
      \item[rule \ruleFuture.] By induction hypothesis,
      there is a formula $\Phi$ such that $\sigma(A) \models
      \Phi$ and $B^F \pperp \Phi$. Since $\sigma \in
      \Sigma_A$, we have $A \models F \Phi$. Let us show
      that $B \pperp F \Phi$. \emph{Ad absurdum}, suppose
      there is $(w,i) \in B$ such that $(w,i) \models F
      \Phi$. Then, there is $j \in [i,|w|]$ such that $(w,j)
      \models \Phi$. By definition of $B^F$, we have $(w,j)
      \in B^F$, in contradiction with $B^F \pperp \Phi$. So,
      $B \pperp F \Phi$.
    \end{description} 
  \end{description}

  ($\Leftarrow$): By structural induction on $\Phi$.  
  \begin{description}
    \item[base case: $\Phi$ literal.] 
      In this case, the derivation tree is a simple
      \ruleAtomic axiom. 
    \item[induction step: $\Phi = \Phi_1 \lor \Phi_2$.] 
      Let $A_1 \coloneqq \{ a \in A : a \models \Phi_1 \}$
      and $A_2 \coloneqq A \setminus A_1$. From $A \models
      \Phi$ we get $A_1 \models \Phi_1$ and $A_2 \models
      \Phi_2$. From $B \pperp \Phi$ we get $B \pperp \Phi_1$
      and $B \pperp \Phi_2$. Since $A_i \models \Phi_i$ and
      $B \pperp \Phi_i$ for both $i \in \{1,2\}$, by
      induction hypothesis there are derivation trees for
      $(A_i,B)$ of size $|\Phi_i|$. With an application of
      the rule \ruleAnd we then obtain a derivation tree for
      $(A,B)$ of size $|\Phi_1| + |\Phi_2| + 1 = |\Phi| =
      k$.
    \item[induction step: $\Phi = \Phi_1 \land \Phi_2$.] 
      Let $B_1 \coloneqq \{ a \in B : a \not\models \Phi_1
      \}$ and $B_2 \coloneqq B \setminus B_1$. From $B
      \pperp \Phi$ we get $B_1 \pperp \Phi_1$ and $B_2
      \pperp \Phi_2$. From $A \models \Phi$ we get $A
      \models \Phi_1$ and $A \models \Phi_2$. Since $A
      \models \Phi_i$ and $B_i \pperp \Phi_i$ for both $i
      \in \{1,2\}$, by induction hypothesis there are
      derivation trees for $(A,B_i)$ of size $|\Phi_i|$.
      With an application of the rule \ruleOr we then obtain
      a derivation tree for $(A,B)$ of size $|\Phi_1| +
      |\Phi_2| + 1 = |\Phi| = k$.
    \item[induction step: $\Phi = X \Psi$.] 
      Since $A \models X \Psi$, for every $(w,i) \in A$ we
      have $i < |w|$ and  $(w,i+1) \models \Psi$. Then,
      $|A^X| = |A|$ and $A^X \models \Psi$, by definition of
      $A^X$. Similarly, from $B \pperp X \Psi$, for every
      $(u,j) \in B$, either $j = |u|$ or $(u,j+1)
      \not\models \Psi$. Hence, $B^X \pperp \Psi$. By
      induction hypothesis, there is a derivation tree for
      $(A^X,B^X)$ of size $|\Psi|$, and by applying the rule
      \ruleNext we obtain a derivation tree for $(A,B)$ of
      size $|\Psi|+1 = |\Phi| = k$.
    \item[induction step: $\Phi = F \Psi$.] 
      Since $A \models F \Psi$, for every $a = (w,i) \in A$
      there is $j_a \in [1,|w|]$ such that $(w,j_a) \models
      \Psi$. Let $\sigma \in \Sigma_A$ be the map given by
      $\sigma(w,i) = j_{(w_i)}$. We have $\sigma(A) \models
      \Psi$. We show that $B^F \pperp \Psi$. \emph{Ad
      absurdum}, suppose there is $(w,j) \in B^F$ such that
      $(w,j) \models \Psi$. By definition of $B^F$ there is
      $i \leq j$ such that $(w,i) \in B$, and we have $(w,i)
      \models F \Psi$. This contradicts the fact that $B
      \pperp F \Psi$. By induction hypothesis, there is a
      derivation tree for $(\sigma(A),B^F)$ of size
      $|\Psi|$. By applying the rule \ruleFuture we obtain a
      derivation tree for $(A,B)$ of size $|\Psi|+1 = |\Phi|
      = k$. 
      \qedhere
  \end{description}
\end{proof}

\begin{corollary}
  Let $\Phi$ be in cosafety LTL(X,F), and $(A,B)$ such that
  $A \models \Phi$ and $B \pperp \Phi$. If all derivation
  trees of $(A,B)$ have size greater than $k$, then $|\Phi|
  \geq k$.
\end{corollary}

\begin{lemma}
  \label{lemma:monotonicity-B}
  If all derivation trees of $(A,B)$ have size greater than
  $k$, then for every $C$, all derivation trees of $(A,B
  \cup C)$ and $(A \cup C, B)$ have size greater than $k$.
\end{lemma}

\begin{proof}
  We prove the statement involving $(A,B \cup C)$. The case
  of $(A \cup C, B)$ is analogous. We show the
  contrapositive statement, i.e., if there is $C$ such that
  $(A,B \cup C)$ has a derivation tree of size at most $k$,
  then $(A,B)$ has a derivation tree of size at most $k$.
  The proof is by induction on the structure of the
  derivation tree, and by cases depending on the rule used
  at the root of the tree.
  \begin{description}
    \item[base case: \ruleAtomic.] 
      In this case we have $A \models \alpha$ and $(B \cup
      C) \pperp \alpha$ for some literal $\alpha$. Hence, $B
      \pperp \alpha$, which implies that $(A,B)$ has a
      derivation tree of size $1$.

    \item[induction step: \ruleOr.] 
      There are $A_1$ and $A_2$ such that $A = A_1 \uplus
      A_2$ and $(A_1,B \cup C)$ and $(A_2,B \cup C)$ have
      derivation trees of size $k_1$ and $k_2$,
      respectively, with $k_1 + k_2 \leq k-1$. By induction
      hypothesis, $(A_1,B)$ and $(A_2,B)$ have derivation
      trees of size at most $k_1$ and $k_2$. By applying the
      rule \ruleOr, we conclude that $(A,B)$ has a
      derivation tree of size at most $k_1 + k_2 + 1 \leq
      k$.

    \item[induction step: \ruleAnd.] 
      There are $B_1,B_2,C_1,C_2$ such that $B = B_1 \uplus
      B_2$, $C = C_1 \uplus C_2$, and $B = (B_1 \cup C_1)
      \uplus (B_2 \cup C_2)$, and moreover $(A,B_1 \cup
      C_1)$ and $(A,B_2 \cup C_2)$ have derivation trees of
      size $k_1$ and $k_2$, respectively, with $k_1 + k_2
      \leq k-1$. By induction hypothesis, $(A,B_1)$ and
      $(A,B_2)$ have derivation trees of size at most $k_1$
      and $k_2$. By applying the rule \ruleAnd, we conclude
      that $(A,B)$ has a derivation tree of size at most
      $k_1 + k_2 + 1 \leq k$. 

    \item[induction step: \ruleNext.] 
      We have $|A^X| = |A|$ and the pair $(A^X,(B \cup
      C)^X)$ has a derivation tree of size at most $k-1$.
      Note that $(B \cup C)^X = B^X \cup C^X$, by definition
      of $(\cdot)^X$. Hence, by induction hypothesis,
      $(A^X,B^X)$ has a derivation tree of size at most
      $k-1$. By applying the rule \ruleNext we conclude that
      $(A,B)$ has a derivation tree of size at most $k$.
      
    \item[induction step: \ruleFuture.] 
      There is $\sigma \in \Sigma_A$ such that
      $(\sigma(A),(B \cup C)^F)$ has a derivation tree of
      size at most $k-1$. Note that $(B \cup C)^F = B^F \cup
      C^F$, by definition of $(\cdot)^F$. Hence, by
      induction hypothesis, $(\sigma(A),B^F)$ has a
      derivation tree of size at most $k-1$. By applying the
      rule \ruleFuture we conclude that $(A,B)$ has a
      derivation tree of size at most $k$.
  \end{description}
  As already said, the proof of the case $(A \cup C, B)$
  follows with a similar proof. There, one notes that $|(A
  \cup C)^X| = |A \cup C|$ implies $|A^X| = |A|$ by
  definition of $(\cdot)^X$, which is required to carry out
  the proof for the \ruleNext rule, and that $\sigma(A \cup
  C) = \sigma(A) \cup \sigma(C)$ by definition of $\sigma
  \in \Sigma_A$, which is required to carry out the proof
  for the \ruleFuture rule.
\end{proof}

The rule for \ruleUntil is more involved. A map $\mu \colon
\Sigma_A \times A \to \N$ is said to be an \emph{until
refutation} for $A$ whenever $i \leq \mu(\sigma,w,i) \leq
\sigma(w,i)$ for every $(w,i) \in A$ and $\sigma \in
\Sigma_A$. Let $\Pi_{A}$ be the set of all until refutation
for $A$. Given $\sigma \in \Sigma_A$, we define
$(\sigma,A)^{\forall U} \coloneqq \{(w,j) : (w,i) \in A,\, i
\leq j < \sigma(w,i)\}$. Let $\mu(B)^{\forall} \coloneqq \{
(w,\mu(\sigma,w,i)) : (w,i) \in B,\, \sigma \in \Sigma_B,\,
\mu(\sigma,w,i) < \sigma(w,i)\}$ and $\mu(B)^{\exists}
\coloneqq \{ (w,\mu(\sigma,w,i)) : (w,i) \in B,\, \sigma \in
\Sigma_B,\, \mu(\sigma,w,i) = \sigma(w,i) \}$


\begin{mathpar} 
  \inferrule[\ruleUntil]{((\sigma,A)^{\forall
  U},\mu(B)^\forall) \and (\sigma(A),\mu(B)^\exists) \and
  \sigma \in \Sigma_A \and \mu \in \Pi_B}{(A,B)}
\end{mathpar}

\begin{theorem}
  The pair $(A,B)$ has a derivation tree of size $k$ if and
  only if there is a formula~$\Phi$ of cosafety LTL of size
  $k$ such that $A \models \Phi$ and $B \models \lnot \Phi$.
\end{theorem}


\begin{lemma}
  \label{lemma:all-pairs-are-considered}
  Consider a (non-closed) derivation tree having $(A,B)$ as
  a root, and such that only the rules \ruleAnd and \ruleOr
  are used. Then, for every $a \in A$ and $b \in B$ there is
  a leaf $(A',B')$ of the tree such that $a \in A'$ and $b
  \in B'$.
\end{lemma}

\begin{proof}
  Trivial induction on the size of the tree.
\end{proof}

\section{Example}

For simplicity, instead of pairs $(w,i)$ let us just keep
the suffix of the word starting at $i$. We will also assume
that every position in the word satisfies exactly one
propositional symbol. Let $A = \{ abb, aaa \}$ and $B = \{
baa , aba \}$. A possible derivation tree for $(A,B)$ is
given by: 
\begin{mathpar} 
  \inferrule*[Right = \ruleAnd]{ \inferrule*[Right =
    \ruleAtomic]{\{abb,aaa\} \models a \and \{baa\} \pperp
    a}{(\{abb,aaa\},\{baa\})}
    \and 
    \qquad
    (\star)
    \quad
  }{(A,B)}
\end{mathpar}
where $(\star)$ stands for the following derivation of
$(\{abb,aaa\},\{aba\})$:
\begin{mathpar} 
  \inferrule*[Right = \ruleOr]{ \inferrule*[Right =
    \ruleNext]{ \inferrule*[Right = \ruleNext]{
    \inferrule*[Right = \ruleAtomic]{ \{b\} \models b 
          \and 
          \{a\} \pperp b }{(\{b\},\{a\})} }{(\{bb\},\{ba\})}
        }{(\{abb\},\{aba\})}
    \and 
    \qquad
    \inferrule*[Right = \ruleNext]{ \inferrule*[Right =
      \ruleAtomic]{ \{a\} \models a 
        \and 
        \{b\} \pperp a }{(\{aa\},\{ba\})}
      }{(\{aaa\},\{aba\})}
    \quad
  }{(\{abb,aaa\},\{aba\})}
\end{mathpar}

This derivation tree for $(A,B)$ has size 8, and corresponds
to the formula $a \land ( XX b \lor X a )$.

However, a derivation tree of size 7 can be found by
changing the derivation of $(\star)$ to
\begin{mathpar} 
  \inferrule*[Right = \ruleNext]{ \inferrule*[Right =
    \ruleOr]{ \inferrule*[Right = \ruleNext]{
    \inferrule*[Right = \ruleAtomic]{ \{b\} \models b 
            \and 
            \{a\} \pperp b }{(\{b\},\{a\})}
          }{(\{bb\},\{ba\})} \and\and \inferrule*[Right =
          \ruleAtomic]{ \{a\} \models a 
        \and 
        \{b\} \pperp a }{(\{aa\},\{ba\})}
      }{(\{bb,aa\},\{ba\})} }{(\{abb,aaa\},\{aba\})}
\end{mathpar}
This shows that $(A,B)$ is separated by the formula $a \land
X ( X b \lor a)$; which is clearly equivalent to the
previous one. Another separating formula of size $8$ is $XX
b \lor (a \land X a)$; note that this formula is not
equivalent to the previous two.

Another remark. Note that the pair $(\{a\},\{ab\})$ does not
have any derivation tree, because none of the rules can be
applied to this pair (here we are excluding the \ruleUntil
rule; with that rule we get a cyclic behaviour that still
does not allow to close the tree). As a consequence, we
obtain that for every $\Phi$ of cosafety LTL(X,F), $a
\models \Phi$ if and only if $ab \models \Phi$, which is
clearly true since cosafety languages are closed under
adding suffixes.  

\section{Connections with learning}

There are a few proposals on how to learn LTL formulae from
positive and negative examples. See
e.g.~\cite{Neider18,Fijalkow21}. It would be nice to see if
these algorithms can be seen as strategies to build proofs
in the above proof system.

\section{Sub-additive proof measures for propositional logic}

In~\cite{Hella12} Hella and V\"a\"an\"anen used a
game-theoretic view of the proof system restricted to the
axiom \ruleAtomic and rules \ruleAnd and \ruleOr to show a
quadratic lower-bound for Parity on propositional formulae.
Their approach is interesting, because they tame the
combinatorics of \ruleAnd and \ruleOr by designing a
suitable function based on the Hamming distance. In this
section we abstract away from the particular function and
show that, as long as one finds a sub-additive function, the
result follows. A similar technique is used
in~\cite{Ueno13}, with interesting applications to LP.

Let $\Pi$ be the set of all pairs of set of structures
$(A,B)$ over which the proof system works. We say that a map
$\mu \colon \Pi \to \{ r \in \R : r > 0\}$ is a
\emph{sub-additive proof measure for $\Pi$} whenever it
satisfies the following properties: 
\begin{enumerate}
  \item given $A,B$ non-empty, if \ruleAtomic can be applied
  to $(A,B)$ then $\mu(A,B) \leq \min(|A|,|B|)$,
  \item for every $A_1,A_2$ such that $A = A_1 \uplus A_2$,
  we have $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$,
  \item for every $B_1,B_2$ such that $B = B_1 \uplus B_2$,
  we have $\mu(A,B) \leq \mu(A,B_1) + \mu(A,B_2)$. 
\end{enumerate}

\begin{theorem}
  \label{lemma:Hella:minimal-tree}
  Let $\mu$ be a sub-additive proof measure for $\Pi$, and
  $(A,B) \in \Pi$ with $A$ and $B$ non-empty. Every
  derivation tree for $(A,B)$ has size at least
  $\frac{\mu(A,B)^2}{|A| \cdot |B|}$.
\end{theorem}

Before proving~\Cref{lemma:Hella:minimal-tree} we need the
following result.
\begin{lemma}
  \label{lemma:Hella:and-or}
  Let $\mu$ be a sub-additive proof measure. Then,
    \begin{itemize}
      \item Let $A_1,A_2$ non-empty such that $A = A_1
      \uplus A_2$. Then, $\frac{\mu(A_1,B)^2}{|A_1|} +
      \frac{\mu(A_2,B)^2}{|A_2|} \geq
      \frac{\mu(A,B)^2}{|A|}$.
      \item Let $B_1,B_2$ non-empty such that $B = B_1
      \uplus B_2$. Then, $\frac{\mu(A,B_1)^2}{|B_1|} +
      \frac{\mu(A,B_2)^2}{|B_2|} \geq
      \frac{\mu(A,B)^2}{|B|}$.
    \end{itemize}
\end{lemma}

\begin{proof}
  We prove the first item. The proof of the second item is
  analogous. Given real numbers $x_1,x_2,w_1,w_2 > 0$,
  recall that the weighted harmonic and arithmetic means are
  defined as: 
  \begin{align}
    H \coloneqq \frac{w_1+w_2}{\frac{w_1}{x_1} + \frac{w_2}{x_2}} \tag{weighted harmonic mean}\\
    A \coloneqq \frac{w_1 \cdot x_1 + w_2 \cdot x_2}{w_1+w_2}
    \tag{weigthed arithmetic mean}
  \end{align}
  It is a well known fact that the former mean is always
  upper bounded by the latter, i.e., $H \leq A$ :
  \begin{align}
    \frac{A}{H} 
      &= \frac{w_1 \cdot x_1 + w_2 \cdot x_2}{w_1+w_2} \cdot \frac{\frac{w_1}{x_1} + \frac{w_2}{x_2}}{w_1 + w_2}\\
      &= \frac{1}{(w_1+w_2)^2} 
        \cdot (w_1 \cdot x_1 + w_2 \cdot x_2) 
        \cdot \left(\frac{w_1}{x_1} + \frac{w_2}{x_2}\right)\\
      &\geq \frac{1}{(w_1+w_2)^2}  \cdot \left(
        \sqrt{w_1 \cdot x_1} \cdot \sqrt{\frac{w_1}{x_1}} + 
        \sqrt{w_2 \cdot x_2} \cdot \sqrt{\frac{w_2}{x_2}} 
        \right)^2 
      & \text{Cauchy--Schwarz inequality}\\
      & = \frac{(w_1+w_2)^2}{(w_1+w_2)^2} = 1.
  \end{align}
  Then, the result follows using the fact that $|A| = |A_1|
  + |A_2|$ and $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$:

  \begin{align}
    \frac{\frac{\mu(A_1,B)^2}{|A_1|} +\frac{\mu(A_2,B)^2}{|A_2|}}{\mu(A,B)} 
    & 
    \geq \frac{\frac{\mu(A_1,B)^2}{|A_1|} +\frac{\mu(A_2,B)^2}{|A_2|}}{\mu(A_1,B) + \mu(A_2,B)}
    &\text{by $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$}
    \\[3pt]
    &
    \geq \frac{\mu(A_1,B) + \mu(A_2,B)}{|A_1| + |A_2|}
    &\text{from } \frac{1}{H} \geq \frac{1}{A}\\ 
    &\geq \frac{\mu(A,B)}{|A|} 
      &\text{by $|A| = |A_1| + |A_2|$ and}\\[-7pt]
    &&\text{by $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B).$}
    &\qedhere
  \end{align}
\end{proof}

\begin{proof}[Proof of~\Cref{lemma:Hella:minimal-tree}]
  We prove that for every $n \in \N$, if $(A,B)$ has a
  derivation tree of size $n$ then $n \geq
  \frac{\mu(A,B)^2}{|A| \cdot |B|}$. The proof is by
  induction on $n$.

  \begin{description}
    \item[base case: $n = 1$.] 
    Since $n = 1$, the derivation tree of $(A,B)$ must be a
    simple application of the axiom \ruleAtomic. Since $\mu$
    is a sub-additive proof measure, and $A$ and $B$ are
    non-empty, $\mu(A,B) \leq \min(|A|,|B|)$, and therefore
    $\frac{\mu(A,B)^2}{|A| \cdot |B|} \leq 1 = n$.

    \item[induction step: $n \geq 2$.] 
    Consider a derivation tree for $(A,B)$ having size $n
    \geq 2$, and observe the rule used at the root of the
    tree, i.e., the root rule. Since $n \geq 2$, the rule is
    either \ruleOr or~\ruleAnd.  
    We show that $n \geq \frac{\mu(A,B)^2}{|A| \cdot |B|}$
    for the case where the root rule is \ruleOr. The case of
    \ruleAnd is analogous.

    Let $A_1,A_2$, such that $A = A_1 \uplus A_2$, be the
    two sets considered by the root rule \ruleOr, and $n_1
    \in \N$ and $n_2 \in \N$ be the size of the derivation
    trees for $(A_1,B)$ and $(A_2,B)$. Note that we can
    assume both $A_1$ and $A_2$ to be non-empty, otherwise
    we would have $A = A_1$ or $A = A_2$ and one can modify
    the derivation tree to find a proof for $(A,B)$ of size
    $n' < n$; and obtain $n \geq \frac{\mu(A,B)^2}{|A| \cdot
    |B|}$ by induction hypothesis. So, under the assumption
    that $A_1$ and $A_2$ are non-empty, we have
    \begin{align}
      n & > n_1 + n_2 
          &\text{by definition}\\ 
        & \geq \frac{\mu(A_1,B)^2}{|A_1| \cdot |B|} + \frac{\mu(A_2,B)^2}{|A_2| \cdot |B|}
          &\text{by induction hypothesis}\\ 
        & = \frac{1}{|B|} \cdot \left( \frac{\mu(A_1,B)^2}{|A_1|} + \frac{\mu(A_2,B)^2}{|A_2|}\right)\\
        & \geq \frac{\mu(A,B)^2}{|A| \cdot |B|}
          &\text{by~\Cref{lemma:Hella:and-or}.} 
          &\qedhere
    \end{align}
  \end{description}
\end{proof}

We now show how to
instantiate~\Cref{lemma:Hella:minimal-tree} to obtain a
quadratic lower bound for the size of the formula expressing
parity. For simplicity, we consider $A,B \subseteq
\{0,1\}^k$ encoding sets of truth assignments to the
propositional symbols $\{p_0,\dots,p_{k-1}\}$. Define
$\delta_1 \colon \Pi \to \N$ to be the function:
\[
  \delta_1(A,B) \coloneqq \max(1,|\{ (a,b) \in A \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \}|).
\] 


\begin{lemma}
  \label{lemma:Hella:delta1proofmeasure}
  The function $\delta_1$ is a sub-additive proof measure.
\end{lemma}

\begin{proof}
  (1) We show the contrapositive of the first requirement of
  a sub-additive proof measure: given $A,B$ non-empty, if
  $\delta_1(A,B) > \min(|A|,|B|)$, then the axiom
  \ruleAtomic cannot be applied. Suppose $\min(|A|,|B|) =
  |A|$ (the case for $|B| = \min(|A|,|B|$) is analogous). We
  have $\delta_1(A,B) > |A|$ and so there is $a \in A$ and
  two distinct $b_1,b_2 \in B$ having Hamming distance $1$
  from $a$. Hence, for every $i \in [0,k-1]$, we have $a[i]
  = 1 \Leftrightarrow b_1[i] = 1$ or $a[i] = 1
  \Leftrightarrow b_2[i] = 1$. This implies that \ruleAtomic
  cannot be used for $p_i$ nor for $\lnot p_i$ (for all $i
  \in [0,k-1]$).

  (2) We show that $\delta_1(A,B) \leq \delta_1(A_1,B) +
  \delta_1(A_2,B)$, for all $A_1,A_2$ such that $A = A_1
  \uplus A_2$. Let, 
  \begin{align} 
    \Delta &\coloneqq \{ (a,b) \in A \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \},\\ 
    \Delta_1 &\coloneqq
    \{ (a,b) \in A_1 \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \},\\ 
    \Delta_2 &\coloneqq
    \{ (a,b) \in A_2 \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \}.
  \end{align}
  Note that, by definition, $\Delta = \Delta_1 \uplus
  \Delta_2$. If $\Delta_1$ or $\Delta_2$ are empty, then
  either $\Delta = \Delta_1$ or $\Delta = \Delta_2$, and
  thus $\delta_1(A,B) \leq \delta_1(A,B) + 1 =
  \delta_1(A_1,B) + \delta_1(A_2,B)$ follows by definition
  of $\delta_1$. Otherwise, $\Delta_1$ and $\Delta_2$ are
  non-empty and thus $\delta_1(A,B) = |\Delta| = |\Delta_1|
  + |\Delta_2| = \delta_1(A,B) + \delta_2(A,B)$, as
  required.

  (3) the proof that $\delta_1(A,B) \leq \delta_1(A,B_1) +
  \delta_1(A,B_2)$, for every $B_1,B_2$ such that $B = B_1
  \uplus B_2$, follow similarly to the previous point. 
\end{proof}


\begin{corollary}
  Let $k \geq 1$. If $\Phi$ is a propositional formula
  expressing the parity of strings $s \in \{0, 1\}^k$, then
  the size of $\Phi$ is at least $k^2$.
\end{corollary}

\begin{proof}
  Let $A \coloneqq \{ s \in \{0, 1\}^k : s \text{ has an odd
  number of $1$s} \}$ and $B \coloneqq \{0,1\}^k \setminus
  A$. Therefore, $|A| = |B| = 2^{k-1}$. For every $a \in A$,
  there are exactly $k$ different $b \in B$ having Hamming
  distance $1$ from $a$. Then, $\delta_1(A,B) = k \cdot
  2^{k-1}$ and by~\Cref{lemma:Hella:minimal-tree}
  and~\Cref{lemma:Hella:delta1proofmeasure} we conclude that
  the minimal derivation tree for $(A,B)$ as size at least
  $\frac{\delta_1(A,B)^2}{|A| \cdot |B| } = k^2$.
\end{proof}

\section{Sub-additive proof measures, version 2}
In fact, the definition below is a generalization of the one
in the previous section that works well for infinite models.

Let $\Pi$ be the set of all pairs of set of structures
$(A,B)$ over which the proof system works. We say that a map
$\mu \colon \Pi \to \{ r \in \R : r > 0\}$ is a
\emph{sub-additive proof measure for $\Pi$} whenever it
satisfies the following properties: 
\begin{enumerate}
  \item given $A,B$ non-empty, if \ruleAtomic can be applied
  to $(A,B)$ then $\mu(A,B) \leq 1$,
  \item for every $A_1,A_2$ such that $A = A_1 \uplus A_2$,
  we have $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$,
  \item for every $B_1,B_2$ such that $B = B_1 \uplus B_2$,
  we have $\mu(A,B) \leq \mu(A,B_1) + \mu(A,B_2)$. 
\end{enumerate}

\begin{theorem}
  \label{lemma:Hella:minimal-tree-two}
  Let $\mu$ be a sub-additive proof measure for $\Pi$, and
  $(A,B) \in \Pi$ with $A$ and $B$ non-empty. Every
  derivation tree for $(A,B)$ has size at least $\mu(A,B)$.
\end{theorem}

Indeed, given a proof measure $\mu'$ defined as in the
previous section, setting $\mu(A,B) \coloneqq
\frac{\mu'(A,B)^2}{|A| \cdot |B|}$ allows us to obtain a
sub-additive proof measure w.r.t.~the above three
conditions.

For \ruleNext and \ruleFuture it seems we could add
something like: 
\begin{enumerate}
  \item[4.] $\mu(A,B) \leq \mu(A^X,B^X) + f(|A|)$ 
\end{enumerate}
where $f \colon \N \to \{ r \in \R : r \geq 0 \}$ is a fixed
monotone function. Then the theorem would become that the
minimal derivation tree of $(A,B)$ has size
$\frac{\mu(A,B)}{f(|A|)}$. So, $f$ should grow slower than
$\mu$ if we want something nice.

\section{Could this work?}
We do not consider the \ruleUntil rule. Consider two
disjoint families of propositional symbols $P =
\{p_1,\dots,p_n\}$ and $Q = \{q_1,\dots,q_n\}$, with $n \geq
2$. We look at the following formula: 
\[ 
  \Phi_n \coloneqq F\left( \bigvee_{j=1}^n q_j \land \bigwedge_{i=1}^n 
    \Big( 
      (q_i \land F^{-1}{p_i}) 
      \lor
      \big(\lnot q_i \land F^{-1}(\lnot p_i \land \bigvee_{j=1}^n p_j)\big)
    \Big)
  \right).
\]
We consider infinite words over the alphabet $2^{P \cup Q}$.
Let $T_P \coloneqq 2^P \setminus \{\emptyset\}$. Given a set
$\tau \in T_P$, we write $\tau^Q$ for the set in $T_Q
\coloneqq 2^P \setminus \{\emptyset\}$ obtained from $\tau$
by replacing $p_i$ with $q_i$, for every $i \in [1,n]$.

Let $E_Q \in (T_Q)^*$ be a finite word enumerating all
elements in $T_Q$. Given a subset $S \subseteq T_Q$, we
write $E_Q|_{-S}$ for the restriction of $E_Q$ to elements
not in $S$, which maintain the same ordering with respect to
the enumeration. For instance, for $Q = \{q_1,q_2\}$, we
might have $E_Q = \{q_1\} \cdot \{q_2\} \cdot \{q_1,q_2\}$
and given $S = \{ \{q_2\}\}$, $E_Q|_{-S} =  \{q_1\} \cdot
\{q_1,q_2\}$. Lastly, given $\tau \in T_p$, we write
$a(\tau)$ and $b(\tau)$ for the words $a(\tau) \coloneqq
\tau \cdot \emptyset^{2^n} \cdot (E_Q)^\omega$ and $b(\tau)
\coloneqq  \tau \cdot \emptyset^{2^n} \cdot
\left(E_Q|_{-\{\tau^Q\}}\right)^\omega$. 

\begin{lemma}
  Consider $j,k_1,\dots,k_n \in \N$ as well
  as distinct sets ${\rho_1,\dots,\rho_n \in T_Q}$, for some $n \in \N$. 
  Let $a
  \coloneqq (E_Q)^\omega$, $A \coloneqq \{ (a, j) \}$ and $B
  \coloneqq \{\left(\left(E_Q|_{-\{\rho_i\}}\right)^\omega,
  k_i \right) : i \in [1,n] \}$. 
  Let $m$ be the number of $(w,i) \in B$ such that $w[i] = a[j]$.
  Then, the minimal derivation tree of $(A,B)$ has size at least
  $m$.
\end{lemma}

NOTE: I think that $m$ above is essentially a sub-additive proof measure restricted to a particular family of pairs.

\begin{proof}
  If $m = 0$ the statement is
  trivial, as the minimal derivation tree for
  $(A,B)$ needs to be at least an \ruleAtomic rule, and
  has thus size at least $1$. Below, suppose $m \geq 1$. We prove the
  statement by induction on the size of the minimal
  derivation tree. Let~$\mathcal{T}$ be a minimal derivation
  tree for $(A,B)$, and suppose it has size $k$.
  \begin{description}
    \item[base case $k = 1$.] 
      In this case, $\mathcal{T}$ is a simple application of
      the rule~\ruleAtomic. 
      Then, there must be $q \in Q$ such that either $q \in a[j]$ and $q \not \in w[i]$ for every $(w,i) \in B$, or vice versa, i.e.,  $q \not \in a[j]$ and $q \in w[i]$ for every $(w,i) \in B$.
      We conclude that every $(w,i) \in B$ is such that $w[i] \neq a[j]$, and thus $m = 0$ and the statement is proven.
    \item[induction step $k \geq 2$.] 
      We split the proof depending on the rule applied to
      the root $(A,B)$ of $\mathcal{T}$. Note that this rule cannot
      be~\ruleAtomic, since $k \geq 2$.
      \begin{description}
        \item[rule~\ruleOr.] 
          In this case given $A_1,A_2$ such that $A_1 \uplus
          A_2 = A$ we have either $A_1 = A$ or $A_2 = A$.
          This contradicts the minimality of $\mathcal{T}$,
          hence showing that the root of $\mathcal{T}$ is
          not an \ruleOr rule.
        \item[rule \ruleAnd:] 
          Consider $B_1,B_2$ such that $B_1 \uplus B_2 = B$.
          Note that $|B_1| + |B_2| = |B| = n$. 
          Given $\ell \in \{1,2\}$ let $m_\ell$ be the number of $(w,i) \in B_\ell$ such that $w[i] = a[j]$, and let $k_\ell$ be the size of the minimal derivation tree of $(A,B_\ell)$.
          By definition of $B_1$ and $B_2$, $m = m_1 + m_2$ and $k = k_1 + k_2 + 1$. By induction hypothesis, $m_1 \leq k_1$ and $m_2 \leq k_2$, 
          hence $m \leq k_1 + k_2 < k$.
        \item[rule \ruleNext:] 
          the minimal derivation tree for $(A^X,B^X)$ has size $k-1$.
          To conclude that $\mathcal{T}$ has size $m$ it suffices to show that
          the minimal derivation tree for $(A^X,B^X)$ has size at least $m-1$.
          Let $(w_1,i_1),\dots,(w_m,i_m)$ be the $m$ elements of $B$ such that $w_\ell[i_\ell] = a[j]$ for all $\ell \in [1,m]$. 
          By definition, $a[j+1]$ is the successor of $a[j]$ in the enumeration $E_Q$ (where the successor of the last element in $E_Q$ is its first element). \emph{Ad absurdum}, suppose that there are two distinct $\ell,r \in [1,m]$ 
          such that $w_\ell[i_\ell+1] \neq a[j+1]$ and $w_r[i_r+1] \neq a[j+1]$. 
          By definition of $B$ and of $(E_Q|_{-\{\rho_i\}})$, 
          we conclude that $w_\ell = w_r = (E_Q|_{-\{\rho_i\}})^\omega$ for some $i \in [1,n]$. However, each element of $B$ is of the form 
          $\left(\left(E_Q|_{-\{\rho\}}\right)^\omega, k \right)$ for a distinct $\rho \in T_Q$; a contradiction. 
          We conclude that at most one among  $(w_1,i_1+1),\dots,(w_m,i_m+1)$ can be distinct from $a[j+1]$. By definition of $(A^X,B^X)$ and by induction hypothesis, this means that the minimal derivation tree for $(A^X,B^X)$ has size at least $m-1$.
        \item[rule \ruleFuture:]
          Let $\sigma \in \Sigma_A$ be the future point used in this rule. Similarly to the previous case, to conclude the proof it suffices to show that the minimal derivation tree for $(\sigma(A),B^F)$ has size at least $m-1$. In fact, we show that this tree has size at least $n-1$. Note that by definition $m \leq n$. 
          By definition, $\sigma(A) = \{(a,\sigma(a,j))\}$. Let $\rho \coloneqq a[\sigma(a,j)]$. By definition of $B$, there is at most one $(w,i) \in B$ such that $w = (E_Q|_{-\{\rho\}})^\omega$, meaning that $\rho$ appears in at least $n-1$ words in $B$. 
          Therefore, $B^F$ contains at least $n-1$ pairs $(w',i')$ such that $w'[i'] = \rho$. Let $B'$ be a set of $n-1$ such pairs. 
          Since $(\sigma(A),B^F)$ has a derivation tree of size $k-1$, and $B' \subseteq B^F$, we conclude that $(\sigma(A),B')$ has a derivation tree of size at most $k-1$. By induction hypothesis, 
          the minimal derivation tree for $(\sigma(A),B')$ has size at least $n-1$, and therefore the same holds true for $(\sigma(A),B^F)$.
          Here we are relying on the fact that the minimal derivation tree of a pair $(A,B_1)$ is at most the minimal derivation tree of $(A,B_2)$ whenever $B_1 \subseteq B_2$.
          \qedhere
      \end{description}
  \end{description}
\end{proof}

\begin{lemma}
  \label{lemma:lower-bound:trees-with-next-future}
  Let $(A,B)$ containing pairs $\langle a(\tau_i),b(\tau_i)
  \rangle$ for $k$ distinct $\tau_1,\dots,\tau_k \in T_P$.
  Every derivation tree for $(A,B)$ that starts with either
  \ruleNext or \ruleFuture has size at least $k$.
\end{lemma}

\begin{proof}
  Hopefully not too hard to prove...
\end{proof}

We look at the following families: 
\[
  A \coloneqq \{ a(\tau) : \tau \in T_P \},
  \qquad\qquad
  B \coloneqq \{ b(\tau) : \tau \in T_P \}.
\]

\begin{lemma}
  $A \models \Phi_n$ and $B \pperp \Phi_n$.
\end{lemma}

\begin{proof}
  Should be straightforward. 
\end{proof}



\begin{lemma}
  The minimal derivation tree of $(A,B)$ has size at least
  $2^{n}-1$.
\end{lemma}

\begin{proof}
  Let $\mathcal{T}$ be a derivation tree for $(A,B)$. Let
  $\mathcal{T}'$ be the maximal open subtree of
  $\mathcal{T}$ rooted and $(A,B)$, and such that
  $\mathcal{T}'$ only has~\ruleAnd and~\ruleOr nodes. Let
  $L$ be the set of all leafs in $\mathcal{T}'$, and given
  $\ell \in L$, let $[\ell]$ be the number of distinct $\tau
  \in T_P$ such that $\langle a(\tau), b(\tau) \rangle$ is
  contained in $\ell$. If $[\ell] \geq 1$, then the
  rule~\ruleAtomic cannot be used and, together with the
  maximality of $\mathcal{T}'$ we conclude that the
  derivation tree of $\ell$ start with the~\ruleNext or
  the~\ruleFuture rules.
  By~\Cref{lemma:lower-bound:trees-with-next-future}, we
  conclude that the minimal derivation tree for $\ell$ has
  size $[\ell]$, and therefore $\mathcal{T}$ has size at
  least $\sum_{\ell \in L} [\ell]$.
  By~\Cref{lemma:all-pairs-are-considered}, every $\langle
  a(\tau), b(\tau) \rangle$ must be contained in some $\ell
  \in L$, so $\sum_{\ell \in L} [\ell] \geq |T_P| =
  2^{n-1}$.
\end{proof}

\section{Random stuff... (do not read for the moment; it might go in the wrong direction)}

Let's try this formula ($n \geq 2$): 
\[ 
  \Phi_n \coloneqq \exists x : \bigvee_{j=1}^n p_j(x) \land \bigwedge_{i=1}^n (p_i(x) \implies \exists y \leq x : q_i(y))
\]

A few ``guesses'' to reduce the search space: 
\begin{itemize}
  \item instead of positions can satisfy any combination of
  $p_i$s and $q_j$s, maybe it's enough to consider ones that
  satisfy the formula $P_n \coloneqq \bigvee_{j=1}^n p_j
  \land \bigwedge_{j=1}^n \lnot q_j$ or the formula $Q_n
  \coloneqq \bigwedge_{i=1}^n \lnot p_i \land
  \bigvee_{j=1}^n (q_j \land \bigwedge_{k \in [1,n]
  \setminus \{j\}} \lnot q_j)$. E.g., for $n = 3$, the first
  three tuples represent $Q_3$ and the latter $7$ represent
  $P_3$: 
  \begin{align}
    (\lnot p_1,\lnot p_2,\lnot p_3,\mathbf{q_1},\lnot q_2,\lnot q_3)\\
    (\lnot p_1,\lnot p_2,\lnot p_3,\lnot q_1,\mathbf{q_2},\lnot q_3)\\
    (\lnot p_1,\lnot p_2,\lnot p_3,\lnot q_1,\lnot q_2,\mathbf{q_3})\\
    (\mathbf{p_1},\lnot p_2,\lnot p_3,\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\lnot p_1, \mathbf{p_2},\lnot p_3,\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\mathbf{p_1}, \mathbf{p_2},\lnot p_3,\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\lnot p_1,\lnot p_2,\mathbf{p_3},\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\mathbf{p_1},\lnot p_2,\mathbf{p_3},\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\lnot p_1,\mathbf{p_2},\mathbf{p_3},\lnot q_1,\lnot q_2,\lnot q_3)\\
    (\mathbf{p_1},\mathbf{p_2},\mathbf{p_3},\lnot q_1,\lnot q_2,\lnot q_3)\\
  \end{align}
  \item Maybe it is possible for $A$ and $B$ to be picked so
  that only the last position in each word satisfy $P_n$.
  This won't be possible for non-cosafety language, because
  then I can state whether I'm at the last element of the
  word, and then the formula below becomes annoying: 
  \[ 
    \bigvee_{i=1}^n @\text{last}(p_i) \land \bigwedge_{j=1}^n (@\text{last}( \lnot p_i) \lor F q_i)
  \]
  \item Maybe if each position repeats consecutively enough
  times, e.g., $pppppp$ instead of just $p$, then the
  \ruleNext rule can be thrown away. This would make the
  models exponential in size, but still not really
  arbitrary. Alternatively we could for the time being
  simply remove the \ruleNext rule. TODO CHECK BETTER: In
  fact I think \ruleNext can often be avoided for lower
  bounds, because of the axioms $FX \Phi \implies XF \Phi$,
  $X \Phi \lor X \Psi \iff X(\Phi \lor \Psi)$ and $X \Phi
  \land X \Psi \iff X(\Phi \land \Psi)$.
  \item To check: I think that, in fact, Fagin's games only
  work for FO logics that admit putting a formula in Prenex
  form.
  \item Need a hook for induction, but it is difficult with
  the \ruleAnd and \ruleOr rules.
\end{itemize}

A reasonable guess for the sets might be ($R \coloneqq \vec
r_1\dots\vec r_n$ s.t.~$\{\vec r_1\dots\vec r_n\} = Q_n$):

\[
  A = \left\{ 
    \begin{aligned}
    \vec q_1\dots\vec q_n\vec p_1\dots\vec p_n R : \  
    & \vec p_1,\dots,\vec p_n \in P_n,\, \vec q_1,\dots,\vec q_n \in Q_n, 
      \ \vec p_i \subseteq \vec p_{i+1} \text{ for all } i \in [1,n)\\
    & \{\vec q_1,\dots, \vec q_n\} \supseteq \{ \vec q \in Q_n : \vec q \models q_i \text{ for some $i \in [1,n]$ s.t. } \vec p_1 \models p_i\}
    \end{aligned}
  \right\},
\]

\[
  B = \left\{ 
    \begin{aligned}
    \vec q_1\dots\vec q_n\vec p_1\dots\vec p_n R : \  
    & \vec p_1,\dots,\vec p_n \in P_n,\, \vec q_1,\dots,\vec q_n \in Q_n, 
      \ \vec p_i \subseteq \vec p_{i+1} \text{ for all } i \in [1,n)\\
    & \{\vec q_1,\dots, \vec q_n\} \subset \{ \vec q \in Q_n : \vec q \models q_i \text{ for some $i \in [1,n]$ s.t. } \vec p_1 \models p_i\}
    \end{aligned}
  \right\},
\]
Note: maybe $R$ can be dropped. We clearly have $A \models
\Phi_n$ and $B \pperp \Phi_n$. These sets should be studied
w.r.t. cosafety LTL(F), so no \ruleNext or \ruleUntil. To
add \ruleNext, after each letter in a word of $A$ and $B$
add $2^n$ many ``empty letters'', i.e., tuples that do
satisfy any propositional symbols. Whatever proof was done
for cosafety LTL(F) should be now translatable into a proof
for cosafety LTL(X,F). For \ruleUntil I currently have no
clue.


Further random notes: 

% \begin{itemize} \item Maybe the following formula is
%   easier? 
%     \[ 
%       \Phi_n \coloneqq \exists x : \bigvee_{j=1}^n p_j(x) \land \bigwedge_{i=1}^n (p_i(x) \iff \exists y \leq x : q_i(y))
%     \]
%   \item A different version of $A$ and $B$ using the
%   formula above: 
  
%   \[
%     A = \left\{ \begin{aligned} \vec q_1\dots\vec q_n\vec
%       p_1\dots\vec p_n R : \  
%       & \vec p_1,\dots,\vec p_n \in P_n,\, \vec
%         q_1,\dots,\vec q_n \in Q_n, \text{ there is $k \in
%         [1,n]$ such that }\\
%       & \{\vec q_1,\dots, \vec q_n\} = \{ \vec q \in Q_n :
%       \vec q \models q_i \text{ for some $i \in [1,n]$
%       s.t. } \vec p_k \models p_i\} \end{aligned}
%       \right\},
%   \]

%   \[
%     B = \left\{ 
%       \begin{aligned}
%       \vec q_1\dots\vec q_n\vec p_1\dots\vec p_n R : \  
%       & \vec p_1,\dots,\vec p_n \in P_n,\, \vec q_1,\dots,\vec q_n \in Q_n, 
%         \text{ for all $k \in [1,n]$ we have }\\
%       & \{\vec q_1,\dots, \vec q_n\} \neq \{ \vec q \in Q_n : \vec q \models q_i \text{ for some $i \in [1,n]$ s.t. } \vec p_k \models p_i\}
%       \end{aligned}
%     \right\},
%   \]
% \end{itemize}



==> sections/learning.tex <==
%! root=../main.tex

\section{Connections with learning}
\label{sec:learning}

There are a few proposals on how to learn LTL formulae from
positive and negative examples. See
e.g.~\cite{Neider18,Fijalkow21}. It would be nice to see if
these algorithms can be seen as strategies to build proofs
in the above proof system.



==> sections/lowerbound.tex <==
%! root=../main.tex

\section{A difficult property for $\LTL[\tomorrow,\weaktomorrow,\eventually,\always]$}
\label{sec:lbltlxf}

\textcolor{red}{L.G.: se riusciamo a dimostrare il lower
bound esponenziale per \LTLxf, allora abbiamo un
\emph{matching bound} per la traduzione di \LTLxf in passato
(cioè in \pLTL) o equivalentemente in canonical form (cioè
\Falpha): l'algoritmo di KR23 è ottimale. Inoltre segue un
risultato di incomparabilità rispetto alla succintezza:
\LTLxf può essere esponenzialmente più succinto della sua
forma canonica (risultato di questo paper) e viceversa
(TIME23, Markey).}

\noindent
Throughout the section, we consider two disjoint families of
propositional symbols $P = \{p_1,\dots,p_n\}$ and $Q =
\{q_1,\dots,q_n\}$, with $n \geq 2$. We look at the
following formula: 
\[ 
  \Phi_n \coloneqq F\left( \bigvee_{j=1}^n q_j \land \bigwedge_{i=1}^n 
  \Big( 
    (q_i \land F^{-1}{p_i}) 
    \lor
    \big(\lnot q_i \land F^{-1}(\lnot p_i \land \bigvee_{j=1}^n p_j)\big)
  \Big)
  \right).
\]
We consider infinite words over the alphabet $2^{P \cup Q}$.
Let $T_P \coloneqq 2^P \setminus \{\emptyset\}$. Given a set
$\tau \in T_P$, we write $\tau^Q$ for the set in $T_Q
\coloneqq 2^Q \setminus \{\emptyset\}$ obtained from $\tau$
by replacing $p_i$ with $q_i$, for every $i \in [1,n]$.

We fix~$\Enum \in (T_Q)^{2^n-1}$ be a finite word
enumerating all elements in $T_Q$, with respect to a strict
total order~$\prec$ on~$T_Q$. Given $\rho \in T_Q$, we write
$\Enum|_{-\rho}$ for the restriction of $\Enum$ to elements
different from $\rho$, which maintain the same ordering with
respect to the enumeration. For instance, for $Q =
\{q_1,q_2\}$, we might have $\{q_1\} \prec \{q_2\} \prec
\{q_1,q_2\}$, and so $\Enum = \{q_1\} \cdot \{q_2\} \cdot
\{q_1,q_2\}$ and given $\rho = \{q_2\}$, we have
$\Enum|_{-\rho} =  \{q_1\} \cdot \{q_1,q_2\}$.

\begin{lemma}
  \label{lemma:lower-bound:spoon-case}
  Consider $j,k_1,\dots,k_n \in \N$ and distinct sets
  ${\rho_1,\dots,\rho_n \in T_Q}$, for some $n \in \N$. Let
  $a \coloneqq \Enum$, and for $i \in [1,n]$, $b_i \coloneqq
  \Enum|_{-\rho_i}$. Define $A \coloneqq \{(a,j)\}$ and $B
  \coloneqq \{(b_i,\, k_i) : i \in [1,n]\}$. Let $m$ be the
  number of $(b,k) \in B$ such that $b[k] = a[j]$. Every
  deduction tree of $(A,B)$ has size at least~${m+1}$.
\end{lemma}

\am{I think that $m$ above is essentially a (partial)
sub-additive proof measure.}

\begin{proof}
  We prove the statement by induction on the size of the
  minimal deduction tree. Let~$\Tree$ be a minimal
  deduction tree for $(A,B)$, and assume that it has
  size~$s$.
  \begin{description}
    \item[base case $s = 1$.] 
      In this case, $\Tree$ is a simple application of the
      rule~\ruleAtomic, and to establish the lemma we must
      show that $m$ is forced to be $0$. Since~\ruleAtomic
      is used, there must be $q \in Q$ such that either $q
      \in a[j]$ and $q \not \in b[i]$ for every $(b,i) \in
      B$, or vice versa, i.e.,  $q \not \in a[j]$ and $q \in
      b[i]$ for every $(b,i) \in B$. Hence, $b[i] \neq a[j]$
      for every $(b,i) \in B$, which implies $m = 0$.
    \item[induction step $s \geq 2$.] 
      Note that if $m = 0$ or $m = 1$ then the statement is
      trivially satisifed. So let us assume~$m \geq 2$. We
      split the proof depending on the rule applied to the
      root $(A,B)$ of $\Tree$. Note that this rule cannot
      be~\ruleAtomic, since $s \geq 2$.
      \begin{description}
        \item[rule~\ruleOr.] 
          In this case given $A_1,A_2$ such that $A_1 \uplus
          A_2 = A$ we have either $A_1 = A$ or $A_2 = A$.
          This contradicts the minimality of $\Tree$, hence
          showing that the root of $\Tree$ is not an \ruleOr
          rule.
        \item[rule \ruleAnd.] 
          Consider $B_1,B_2$ such that $B_1 \uplus B_2 = B$.
          Similarly to the previous case, if $B_1 = B$ or
          $B_2 = B$ then we reach a contradiction with the
          minimality of $\Tree$. So, assume $B_1 \neq
          \emptyset$ and $B_2 \neq \emptyset$. Note that
          $|B_1| + |B_2| = |B| = n$. Given $\ell \in
          \{1,2\}$ let $m_\ell$ be the number of $(b,i) \in
          B_\ell$ such that $b[i] = a[j]$, and let $s_\ell$
          be the size of the minimal deduction tree of
          $(A,B_\ell)$. By definition of $B_1$ and $B_2$, $m
          = m_1 + m_2$ and $s = s_1 + s_2 + 1$. By induction
          hypothesis, $m_1 + 1 \leq s_1$ and $m_2 + 1 \leq
          s_2$, hence $m+1 \leq s_1 + s_2 - 1 < k$.
        \item[rule \ruleNext.] 
          Remark that in order for~\ruleNext to be
          applicable, there must be the case that
          $|A^{\ltl{X}}| = |A|$, that is $a[j]$ does not
          correspond to the last element in the 
          enumeration~$\Enum$. The minimal deduction tree for
          $(A^{\ltl{X}},B^{\ltl{X}})$ has size $s-1$. To
          conclude that~$\Tree$ has size $m+1$ it suffices
          to show that the minimal deduction tree for
          $(A^{\ltl{X}},B^{\ltl{X}})$ has size at least $m$.
          Let $(b_1,i_1),\dots,(b_m,i_m)$ be the $m$
          elements of $B$ such that $b_\ell[i_\ell] = a[j]$
          for all $\ell \in [1,m]$. By definition, $a[j+1]$
          is the successor of $a[j]$ in the enumeration
          $\Enum$. \emph{Ad absurdum}, suppose that there
          are two distinct $\ell,r \in [1,m]$ such that
          $b_\ell[i_\ell+1] \neq a[j+1]$ and $b_r[i_r+1]
          \neq a[j+1]$. Since $b_\ell[i_\ell] = b_r[i_r] =
          a[j]$, by definition of $B$ and of
          $\Enum|_{-\rho_i}$, this means that $b_\ell = b_r
          = \Enum|_{-\rho_i}$ for some $i \in [1,n]$.
          However, each element of $B$ is of the form
          $\left(\Enum|_{-\rho}, k \right)$ for a distinct
          $\rho \in T_Q$; a contradiction. We conclude that
          at most one among $(b_1,i_1+1),\dots,(b_m,i_m+1)$
          can be distinct from $a[j+1]$. By definition of
          $(A^{\ltl{X}},B^{\ltl{X}})$ and by induction
          hypothesis, this means that the minimal deduction
          tree for $(A^{\ltl{X}},B^{\ltl{X}})$ has size at
          least $m$.
        \item[rule \ruleFuture.]
          Let $f \in \FP_A$ be the future point used in this
          rule. Similarly to the previous case, to conclude
          the proof it suffices to show that the minimal
          deduction tree for $(f(A),B^{\ltl{F}})$ has size
          at least $m$. By definition, $f(A) =
          \{(a,f(a,j))\}$. Let $\rho \coloneqq a[f(a,j)]$.
          By definition of $B$, there is at most one $(b,i)
          \in B$ such that $b = \Enum|_{-\rho}$. Define $B''
          \coloneqq \{ (b,k + r) : (b,k) \in B',\ r \in \N,\
          {b[k+r] = \rho}\}$. Since $b[k] = a[j]$ for every
          $(b,k) \in B'$, and $|B'| = m$, we have $|B''|
          \geq m - 1$. By induction hypothesis, the minimal
          deduction tree for $(f(A),B'')$ has size at least
          $m$. Therefore, since $B'' \subseteq B^{\ltl{F}}$,
          by~\Cref{lemma:weakening-sets} the minimal
          deduction tree for $(f(A),B^{\ltl{F}})$ has size
          at least $m$.
          \qedhere
      \end{description}
  \end{description}
\end{proof}

Given $\tau \in T_P$, we write $a(\tau)$ and $b(\tau)$ for
the words $a(\tau) \coloneqq \tau \cdot \Enum$ and $b(\tau)
\coloneqq  \tau \cdot \Enum|_{-\tau^Q}$. 

\begin{lemma}
  \label{lemma:lower-bound:trees-with-next-future}
  Let $(A,B)$ containing pairs $\langle
  (a(\tau_i),0),(b(\tau_i),0) \rangle$ for $n$ distinct
  $\tau_1,\dots,\tau_n \in T_P$. Every deduction tree for
  $(A,B)$ that starts with either \ruleNext or \ruleFuture
  has size at least $n+1$.
\end{lemma}

\begin{proof}
  The statement is trivial for $n = 0$ (as every deduction
  tree has size at least $1$), so let us assume $n \geq 1$.
  Let $\Tree$ be the minimal deduction tree for $(A,B)$,
  and suppose it has size $s$. We show that $s \geq n+1$. We
  split the proof depending on the rule applied at the root
  of $\Tree$. 
  \begin{description}
    \item[case~\ruleNext.] 
      The minimal deduction tree for
      $(A^{\ltl{X}},B^{\ltl{X}})$ has size $s-1$. Consider
      $(a,1) \in A^{\ltl{X}}$, and note that
      $(\{(a,1)\},B^{\ltl{X}})$ is a pair considered
      in~\Cref{lemma:lower-bound:spoon-case}. Since
      $\tau_1,\dots,\tau_n$ are distinct, by definition  of
      $B$ we conclude that in $B^{\ltl{X}}$ there are at
      least $n-1$ elements $(b,1) \in B^{\ltl{X}}$ such that
      $b[1] = a[1]$. Then, the minimal deduction tree of
      $(\{(a,1)\},B^{\ltl{X}})$ has size at least $n$,
      by~\Cref{lemma:lower-bound:spoon-case}. Since
      $\{(a,1)\} \subseteq A^{\ltl{X}}$,
      by~\Cref{lemma:weakening-sets} we conclude that $s-1
      \geq n$, i.e., $s \geq n+1$.
    \item[case~\ruleFuture.]
      Let $\sigma \in \Sigma_A$ be the future point used in
      this application of~\ruleFuture. The minimal
      deduction tree for $(\sigma(A),B^{\ltl{F}})$ has size
      $s-1$. If for every $(a,0) \in A$, $\sigma((a,0)) =
      0$, then we reach a contradiction with the minimality
      of $\Tree$: we have $\sigma(A) = A$ and $B \subseteq
      B^{\ltl{F}}$, which by~\Cref{lemma:weakening-sets}
      imply that the minimal deduction tree of $(A,B)$ has
      size $s-1$. Therefore, there must be a pair $(a,j) \in
      A$ with $j \geq 1$. Given $i \in [1,n]$, let $\ell_i$
      be defined as follows: if $a[j] \neq \tau_i$, then
      pick $\ell_i$ to be such that $b(\tau_i)[\ell_i] =
      a[j]$, otherwise ($a[j] = \tau_i$) define $\ell_i =
      1$. Let $B' \coloneqq \{(b(\tau_i),\ell_i) : i \in
      [1,n] \}$, and note that $B' \subseteq B^{\ltl{F}}$.
      Since $\tau_1,\dots,\tau_n$ are distinct, by
      definition there are at least $n-1$ elements $(w,\ell)
      \in B'$ such that $w[\ell] = a[j]$.
      By~\Cref{lemma:lower-bound:spoon-case}, the minimal
      deduction tree of $(\{(a,j)\},B')$ has size at least
      $n$. As in the previous case of the proof, we then
      conclude that $s \geq n+1$
      by~\Cref{lemma:weakening-sets}.
      \qedhere
  \end{description}
\end{proof}

\begin{lemma}
  \label{lemma:lower-bound-final}
  Define $A \coloneqq \{ (a(\tau),0) : \tau \in T_P \}$ and
  $B \coloneqq \{ (b(\tau),0) : \tau \in T_P \}$. Then, 
  \begin{enumerate}
    \item\label{lemma:lower-bound-final:item1} $A \models
    \Phi_n$ and $B \pperp \Phi_n$, and
    \item\label{lemma:lower-bound-final:item2} the minimal
    deduction tree of $(A,B)$ has size at least $2^{n}$.
  \end{enumerate}
\end{lemma}

\begin{proof}[Proof of~\Cref{lemma:lower-bound-final}.\ref{lemma:lower-bound-final:item1}]
  Let us first show that $A \models \Phi_n$. Consider $\tau
  \in T_P$ and the trace $(a(\tau),0)$. To show that this
  trace satisfied $\Phi_n$, pick $j \in \N$ such that
  $a(\tau)[j] = \tau^Q$. It is easy to see that 
  \[
    (a(\tau),j) \models \Big(\bigvee_{j=1}^n q_j\Big) \land \bigwedge_{i=1}^n 
    \Big( 
      (q_i \land F^{-1}{p_i}) 
      \lor
      \big(\lnot q_i \land F^{-1}(\lnot p_i \land \bigvee_{j=1}^n p_j)\big)
    \Big).
  \]
  By definition of $T_Q$, this trace satisfies
  $\bigvee_{j=1}^n q_j$. Given $i \in [1,n]$, we have
  $(a(\tau),j) \models q_i$ if and only if $(a(\tau),0)
  \models p_i$. Therefore, the trace also satisfies
  $\bigwedge_{i=1}^n \Big( (q_i \land F^{-1}{p_i}) 
    \lor
    \big(\lnot q_i \land F^{-1}(\lnot p_i \land
  \bigvee_{j=1}^n p_j)\big) \Big)$.

  We move to $B \pperp \Phi_n$. Consider $\tau \in T_P$ and
  the trace $(b(\tau),0)$. Note that, by definition, the
  only position in $b(\tau)$ satisfying $\bigvee_{j=1}^n
  p_j$ is the position $0$. This means that the subformulae
  $p_i$ and $\lnot p_i \land \bigvee_{j=1}^n p_j$ appearing
  in $\Phi_n$ inside the scope of the $F^{-1}$ modality are
  only satisfied by that position. Consider a $j \in
  [0,|b(\tau)|-1]$. We show that 
  \[ 
    (b(\tau),j) \not\models \Big(\bigvee_{j=1}^n q_j\Big) \land \bigwedge_{i=1}^n 
    \Big( 
      (q_i \land F^{-1}{p_i}) 
      \lor
      \big(\lnot q_i \land F^{-1}(\lnot p_i \land \bigvee_{j=1}^n p_j)\big)
    \Big).  
  \]
  We have $(b(\tau),0) \not\models \bigvee_{j=1}^n q_j$, and
  therefore assume $j \geq 1$. Then, $b(\tau)[j] = \rho \in
  T_Q$ such that $\tau^Q \neq \rho$. Then, there must be $i
  \in [1,n]$ such that either $p_i \in \tau$ and $q_i \not
  \in \rho$, or vice versa $p_i \not \in \tau$ and $q_i \in
  \rho$. In the former case we conclude that $(b(\tau),j)
  \not \models \lnot q_i \land F^{-1}(\lnot p_i \land
  \bigvee_{j=1}^n p_j)$, whereas in the latter case
  $(b(\tau),j) \not \models (q_i \land F^{-1}{p_i})$.
\end{proof}

\begin{proof}[Proof of~\Cref{lemma:lower-bound-final}.\ref{lemma:lower-bound-final:item2}]
  Let $\Tree$ be a deduction tree for $(A,B)$. Let $\Tree'$
  be the maximal open subtree of $\Tree$ rooted and $(A,B)$,
  and such that $\Tree'$ only has~\ruleAnd and~\ruleOr
  nodes. Let $L$ be the set of all leafs in $\Tree'$, and
  given $\ell \in L$, let $[\ell]$ be the number of distinct
  $\tau \in T_P$ such that $\langle (a(\tau),0), (b(\tau),0)
  \rangle$ is contained in~$\ell$. If $[\ell] \geq 1$, then
  the rule~\ruleAtomic cannot be used and, together with the
  maximality of $\Tree'$ we conclude that the deduction
  tree of $\ell$ start with the rules~\ruleNext
  or~\ruleFuture.
  By~\Cref{lemma:lower-bound:trees-with-next-future}, we
  conclude that the minimal deduction tree for $\ell$ has
  size $[\ell]+1$, and therefore $\Tree$ has size at least
  $|L| + \sum_{\ell \in L} [\ell]$.
  By~\Cref{lemma:all-pairs-are-considered}, every $\langle
  a(\tau), b(\tau) \rangle$ must be contained in some $\ell
  \in L$, and therefore $\sum_{\ell \in L} [\ell] \geq |T_P|
  = 2^{n}-1$. Since $|L| \geq 1$, this implies that $\Tree$
  as size at least $2^n$.
\end{proof}

As a corollary of~\Cref{th:ps}, and
by~\Cref{lemma:lower-bound-final}, the following result
follows:

\begin{corollary}
  Every formula of~\LTLxf equivalent to $\Phi_n$ has size at
  least $2^n$.
\end{corollary}

\begin{lemma}
  \label{lemma:a-formula-for-Phi-n}
  There is a formula of~\LTLxf
  that is equivalent to $\Phi_n$ and s.t.~$\size(\Phi_n) < 2^{n+2} n^2$.
\end{lemma}
\begin{proof}
  Note that $\Phi_n$ can be expressed in~\LTLxf with a formula
  of size $2^n n (4 + 3 n) -4 n (1 + n)$:
  \[ 
      \bigvee_{\tau \in T_P}
      \Big( 
        \bigwedge_{p \in \tau} F(p \land F(\tau^Q))
        \land 
        \bigwedge_{p \in P \setminus \tau} F((\bigvee_{i=1}^n p_i) \land \lnot p \land F(\tau^Q))
      \Big),
  \]
  where $F(\tau^Q) \coloneqq F(\bigwedge_{q \in \tau^Q} q
  \land \bigwedge_{q \in Q \setminus \tau^Q} \lnot q)$, which
  has size $2 n$. Indeed, in the formula above, the disjunct
  corresponding to $\tau$ has size $|\tau| \cdot (2n + 3) + |P
  \setminus \tau| \cdot (4n+3) + n - 1$; so the formula has
  size {\allowdisplaybreaks
  \begin{align*}
    &
      |T_P| - 1 + \sum_{\tau \in T_P} (|\tau| \cdot (2n + 3) + |Q \setminus \tau| \cdot (4n+3) + n - 1)\\
    =\ & 
      2^n - 1 + \sum_{i=1}^n {n \choose i} \cdot (i \cdot (2n+3) + (n-i) \cdot (4n + 3) + n - 1)\\
    =\ & 
      2^n - 1 + \sum_{i=1}^n {n \choose i} \cdot (4n^2 + 4n -1 -i \cdot 2n)\\
    =\ & 
      2^n - 1 + \sum_{i=1}^n \left( {n \choose i} \cdot (4n^2 + 4n -1) - {n \choose i} \cdot (i \cdot 2n) \right)\\
    =\ & 
      2^n - 1 + (4n^2 + 4n -1) \cdot \sum_{i=1}^n {n \choose i}  - 2n \sum_{i=1}^n i \cdot {n \choose i} \\
    =\ & 
      2^n - 1 + (4n^2 + 4n -1) \cdot (2^n-1)  - 2n \cdot (2^{n-1}n) \\
    % =\ & 
    %   2^n - 1 + 2^{n+2} \cdot n^2 + 2^{n+2}n -2^n -4n^2 - 4n +1  - 2^{n}n^2 \\
    =\ &  2^n n (4 + 3 n) -4 n (1 + n).
  \end{align*}
  } Let $g(n) \coloneqq 2^{n+1}n^2$. Note that, for every $n
  \in \N$, the function $f(n) \coloneqq 2^n n (4 + 3 n) -4 n
  (1 + n)$ is such that $g(n) \leq f(n) \leq 2 \cdot g(n)$.
\end{proof}

\subsection{Version with Globally and Weak Next}

Throughout the section, we consider two disjoint families of
atomic propositions $P = \{p_1,\dots,p_n\}$ and $Q =
\{q_1,\dots,q_n\}$ from $\Sigma$, with $n \geq 2$. We look at the
following formula: 
\[ 
  \Phi_n \coloneqq F\left( \bigvee_{j=1}^n q_j \land \bigwedge_{i=1}^n 
  \Big( 
    (q_i \land F^{-1}{p_i}) 
    \lor
    \big(\lnot q_i \land F^{-1}(\lnot p_i \land \bigvee_{j=1}^n p_j)\big)
  \Big)
  \right).
\]
Throughout the section, let $\alpha(n) \coloneqq 2^{n+2} n^2$, i.e., the upper bound on one of the formulae characterising~$\Phi_n$, according 
to~\Cref{lemma:a-formula-for-Phi-n}.

Throughout the section, we restrict ourselves to traces 
in $\traces(P \cup Q)$, i.e., traces whose positions correspond to elements of $2^{P \cup Q}$.
Let $T_P \coloneqq 2^P \setminus \{\emptyset\}$. 
Given a type
$\tau \in T_P$, we write $\tau^Q$ for the set in $T_Q
\coloneqq 2^Q \setminus \{\emptyset\}$ obtained from $\tau$
by replacing $p_i$ with $q_i$, for every $i \in [1,n]$.



We fix~$\Enum \in (\emptyset^{\alpha(n)} \cdot T_Q)^{2^n-1}
\cdot \emptyset^{\alpha(n)}$ to be a finite word enumerating
all elements in $T_Q$, with respect to a strict total
order~$\prec$ on~$T_Q$. 
Note that, in $\Enum$, between any two elements in $T_Q$
there are $\alpha(n)$ positions of type~$\emptyset$. 
Given $\rho \in T_Q$, we write $\Enum|_{-\rho}$ for the
trace in $(\emptyset^{\alpha(n)} \cdot T_Q)^{2^n-2} \cdot
\emptyset^{\alpha(n)}$ obtained from~$\Enum$ by eliminating
the only position of type $\rho$, together with the
$\alpha(n)$ positions of type $\emptyset$ preceding it. 
For instance, for $Q = \{q_1,q_2\}$, the strict total order
might be $\{q_1\} \prec \{q_2\} \prec \{q_1,q_2\}$, and so
$\Enum = \emptyset^{\alpha(n)} \cdot \{q_1\} \cdot
\emptyset^{\alpha(n)} \cdot \{q_2\} \cdot
\emptyset^{\alpha(n)} \cdot \{q_1,q_2\} \cdot
\emptyset^{\alpha(n)}$ and $\Enum|_{-\{q_2\}} =
\emptyset^{\alpha(n)} \cdot \{q_1\} \cdot
\emptyset^{\alpha(n)} \cdot \{q_1,q_2\} \cdot
\emptyset^{\alpha(n)} $.

\am{TODO: state overall goal.}

Given $a,b \in \traces(P \cup Q)$,
we write $a \approx b$ whenever $a$ and $b$ belong to the language $\emptyset^k \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot (2^Q)^*$ 
for some $k \in \N$ and $\rho \in T_Q$. \am{todo: explain this a bit.}
% Let $A,B \subseteq \traces(Q)$. 
% We define $L(A,E) \coloneqq n + m$ where 
% \begin{itemize}
%   \item $n$ is the cardinality of the set ${\{ (b,r) \in B : (b,r) \approx (a,j) \text{ for some
%   } (a,j) \in A \}}$,
%   \item $m = \min\{ k \in \N : \text{there are } (a,j) \in A \text{ and } (b,r) \in B \text{ s.t. } a^j = \emptyset^k \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \rho' \cdot w \text{ and } b^r = \emptyset^k \cdot \rho' \cdot w \text{ for some } \rho \in T_Q \text{  and } w \in (2^Q)^*\}$.
% \end{itemize}

% \am{I might need to make $\approx$ even stronger. The \ruleNext is difficult. Other try: 
% make $\alpha(n)$ be twice the upper bound. Then $a \approx_s b$ iff $a \in \emptyset^j \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot (2^Q)^*$ and $b \in \emptyset^k \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot (2^Q)^*$ with either $j = k$ or $j,k \geq \alpha(n) -s$. 
% I need to see how this propagates. Note that then $a \approx_s b$ implies $a \approx_{s+1} b$}



\begin{lemma}
  \label{lemma:lower-bound:spoon-case-with-globally}
  Let $J \subseteq \N$ be a finite set, $r_1,\dots,r_m \in \N$,
  and consider distinct sets ${\rho_1,\dots,\rho_m \in T_Q}$. Let $A \coloneqq \{\Enum\sffx{j} : j \in J\}$, and $B
  \coloneqq \{(\Enum|_{-\rho_k})\sffx{r_k} : k \in [1,m]\}$. 
  Let~$C \coloneqq \{ (a,b) \in A \times B : {a \approx b} \}$.
  Suppose that the minimal deduction tree $\Tree$ for $\separ{A,B}$ exists and has size $s \leq \alpha(n)$.
  Then, $s \geq \abs{C}+1$.
\end{lemma}

\noindent
One observation on the statement of this lemma: 
the hypothesis that the sets $\rho_1,\dots,\rho_m$ are distinct implies $\abs{B} < 2^n$. 
By definition of $\approx$, this implies
$\abs{C} < 2^n$, and from $n \geq 2$ we conclude that 
the interval $[\abs{C}+1,\alpha(n)]$ is not empty.

\begin{proof}
  During the proof, we write $\prec$ for the strict total order on elements of $T_Q$ used to construct the trace $\Enum$ enumerating $T_Q$.
  Before proving the lemma, we show a useful property of the elements of $C$.
  \begin{clm}
    \label{claim-rho-prec-rhok}
    Let $(a,b) \in C$ and $k \in [1,m]$ with $b = (\Enum|_{-\rho_k})\sffx{r_k}$. 
    There are $u \in \N$, $\rho \in T_Q$ and $\sigma \in (2^Q)^*$ such that $\rho \prec \rho_k$ and 
    $b = \emptyset^u \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$.
  \end{clm}
  \begin{proofclaim}
    By definition of $\approx$, 
    there are $u \in \N$, $\rho \in T_Q$ and $\sigma,\sigma' \in (2^Q)^*$ 
    such that 
    \[ 
      a = \emptyset^u \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma' 
      \qquad 
      b = \emptyset^u \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma
    \]
    \emph{Ad absurdum}, suppose $\rho_k \preceq \rho$. 
    Since $\rho$ occurs in $b$, by definition of $\Enum|_{-\rho_k}$ we have $\rho \neq \rho_k$, and thus $\rho_k \prec \rho$. Again by definition of $\Enum|_{-\rho_k}$, 
    this implies that $\sigma$ is a suffix of $\Enum$. By definition of~$\Enum$ and from the two equations above, this means $\sigma = \sigma'$ 
    and so $a = b$. However, this contradicts the existence of $\Tree$ by~\Cref{lemma:unclosable-tree-condition} and~\Cref{th:ps}.
    Hence $\rho \prec \rho_k$.
  \end{proofclaim}

  \vspace{5pt}
  \noindent
  Let us go back to the proof 
  of~\Cref{lemma:lower-bound:spoon-case-with-globally}.
  If $J = \emptyset$ or $m = 0$ then the lemma follows trivially. Below, let us assume $J \neq \emptyset$ and $m \geq 1$. We prove the statement by induction on $s$. 

  \proofitem{base case: $s = 1$} 
  In this case, $\Tree$ is a simple application of the rule~\ruleAtomic. This means that for every $a \in A$ and $b \in B$ we have $a[0] \neq b[0]$. By definition of~$\approx$, we derive $C = \emptyset$, and thus $s \geq \abs{C}+1$.

  \proofitem{induction step: $s \geq 2$}
  Note that if $\abs{C} \leq 1$ then the statement follows trivially. Hence, below, we assume $\abs{C} \geq 2$.
  We split the proof depending on the rule applied to
  the root $\separ{A,B}$ of~$\Tree$. Since $s \geq 2$, this rule
  cannot be~\ruleAtomic.
  \begin{itemize}[align=left]
    \setlength{\itemsep}{3pt}
    \item[\textbf{case: rule~{\rm{\ruleOr}}.}] 
      Consider $A_1,A_2$ such that $A_1 \uplus A_2 = A$.
      The cases where $A_1 = A$ or $A_2 = A$ yield a
      contradiction with the minimality of $\Tree$, 
      as one of the hypotheses used to apply the rule~\ruleOr is $\separ{A,B}$ itself. 
      Hence,
      assume $A_1$ and $A_2$ non-empty.
      For $i \in \{1,2\}$, 
      let $s_i$ be the size of the minimal deduction 
      tree of $\separ{A_i,B}$. 
      Let $C_i \coloneqq \{b \in B :
      {b \approx a} \text{ for some
} a \in A_i \}$.
      By induction hypothesis, $s_1 \geq |C_1|+1$ 
      and $s_2 \geq |C_2|+1$.
      By minimality of $\Tree$,
      we have $s = s_1 + s_2 + 1 \geq |C_1|+|C_2|+3$.
      Since $A_1$ and $A_2$
      partition~$A$, and
      by definition of $\approx$, we get
      $|C| \leq |C_1| + |C_2|$. 
      Then, $s \geq |C| + 2$.
    \item[\textbf{case: rule~{\rm{\ruleAnd}}.}] 
      This case is analogous to the previous one. 
      Consider $B_1,B_2$ such that $B_1 \uplus B_2 = B$.
      The cases where $B_1 = B$ or
      $B_2 = B$ yield a contradiction with the
      minimality of $\Tree$. So, assume $B_1 \neq
      \emptyset$ and $B_2 \neq \emptyset$. 
      For $i \in \{1,2\}$, 
      let $s_i$ be the size of the minimal deduction 
      tree of $\separ{A,B_i}$, and define 
      $C_i \coloneqq \{{b \in B_i} :
      {b \approx a} \text{ for some
      } a \in A \}$.
      By induction hypothesis, $s_1 \geq |C_1|+1$ 
      and ${s_2 \geq |C_2|+1}$.
      By minimality of $\Tree$,
      we have $s = s_1 + s_2 + 1 \geq |C_1|+|C_2|+3$.
      Since $B_1$ and $B_2$
      partition~$B$,
      by definition of $\approx$ we get
      $|C| \leq |C_1| + |C_2|$. 
      Then, $s \geq |C| + 2$.
    \item[\textbf{case: rule~{\rm{\ruleNext}} 
      and~{\rm{\ruleWeakNext}}.}] 
      \!\!We consider the~\ruleNext and~\ruleWeakNext rules
      together, as both rely on deriving $\separ{A^{\ltl{X}},B^{\ltl{X}}}$.
      Perhaps surprisingly, their treatment is non-trivial.
      The minimal deduction tree for
      $\separ{A^{\ltl{X}},B^{\ltl{X}}}$ has size $s-1$. 
      Within this deduction tree, consider the maximal partial deduction tree~$\Tree'$ 
      rooted at $\separ{A^{\ltl{X}},B^{\ltl{X}}}$ and made solely 
      of applications of the rules~\ruleAnd,~\ruleOr,~\ruleNext, and~\ruleWeakNext.
      Let $\separ{A_1,B_1},\dots,\separ{A_q,B_q}$ be the leafs of such a tree. 
      Let $i \in [1,q]$.
      In the original tree~$\Tree$, to $\separ{A_i,B_i}$ it is applied a rule different from~\ruleAnd,~\ruleOr,~\ruleNext and~\ruleWeakNext.
      Let~${\xi_i \geq 1}$ be the number of rules \ruleNext and \ruleWeakNext used in the path of $\Tree$ from $\separ{A,B}$ to $\separ{A_i,B_i}$. 
      Note that, from $s \leq \alpha(n)$, we have $\xi_i \leq \alpha(n)$.
      Moreover, we define:
      \begin{align*}
        C_i &\coloneqq \{(a\sffx{\xi_i},b\sffx{\xi_i}) \in A_i \times B_i : {(a,b) \in {A \times B}},\, {a \approx b},\, a\sffx{\xi_i} \approx b\sffx{\xi_i} \},\\
        N_i &\coloneqq \{(a\sffx{\xi_i},b\sffx{\xi_i}) \in A_i \times B_i : {(a,b) \in A \times B},\, {a \approx b},\,
        a\sffx{\xi_i} \not\approx b\sffx{\xi_i} \}.
      \end{align*}
      By induction hypothesis, the minimal 
      deduction tree for $\separ{A_i,B_i}$ 
      has size $s_i \geq \abs{C_i}+1$.
      We now show series of properties on the sets $C_i$ and $N_i$, from which we derive $s \geq \abs{C}+1$.

      \begin{clm}
        \label{proof-lb1:clm1}
        Let $i \in [1,q]$ and $(a,b) \in N_i$. There 
        are $(a',b') \in C$, $u \in [0,\alpha(n)]$, $v \in [1,\alpha(n)]$, $k \in [1,m]$, $\rho \in T_Q$ and $\sigma \sqsubseteq \Enum$ satisfying the following equations:
        \begin{align*}
          a' &\ =\ \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)-v} \cdot a,\\
          b' &\ =\ \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)-v} \cdot b,\\ 
          b'   & \ =\ (\Enum|_{-\rho_k})\sffx{r_k},\\
          a  &\ =\ \emptyset^v \cdot \rho_k \cdot \emptyset^{\alpha(n)-v} \cdot b,\\
          b &\ =\ \emptyset^v \cdot \sigma.
        \end{align*}
        Moreover, $\xi_i = u+1+\alpha(n)-v$.
      \end{clm}
      \begin{proofclaim}
        Since $(a,b) \in N_i$, there is $(a',b') \in A \times B$ such that $a'\sffx{\xi_i} = a$ and
        $b'\sffx{\xi_i} = b$, and $a' \approx b'$. By definition of $\approx$ and $\Enum$, there are $u \in [0,\alpha(n)]$, $\rho \in T_Q$ and $\mu,\sigma \in (2^Q)^*$ such that 
        $a' =  \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \mu$
        and 
        $b' =  \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$.
        By definition of $A$ and $B$, there is $j \in J$ and $k \in [1,m]$ such that $a' = \Enum\sffx{j}$ and $b' = (\Enum|_{-\rho_k})\sffx{r_k}$; hence $\mu$ and $\sigma$ are suffixes of $\Enum\sffx{j}$ and $(\Enum|_{-\rho_k})\sffx{r_k}$, respectively. Since $\separ{A,B}$ is derivable in the proof system, by~\Cref{lemma:unclosable-tree-condition} and~\Cref{th:ps} we also have $a' \neq b'$.
        The deduction tree $\Tree$ has size $s \leq \alpha(n)$ and 
        the only rules applied to $\Tree'$ are~\ruleAnd,~\ruleOr,~\ruleNext and~\ruleWeakNext. 
        Because of this, one of the following two cases hold: 
        \begin{enumerate}
          \item $a = \emptyset^{t} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \mu$ and $b = \emptyset^{t} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$, for some $t < u$, or 
          \item there is $v \in [1,\alpha(n)]$ such that $a = \emptyset^{v} \cdot \mu$ and $b = \emptyset^{v} \cdot \sigma$.
        \end{enumerate}
        However, in the first case one derives $a \approx b$, in contradiction with $(a,b) \in N_i$. 
        We are thus in the second case. 
        Then, from the fact that $a \not\approx b$, and $\mu$ and $\sigma$ are suffixes of $\Enum$ and $(\Enum|_{-\rho_k})\sffx{r_k}$, we conclude that $\mu = \rho_k \cdot \emptyset^{\alpha(n)} \cdot \sigma$. Putting together all equations derived until now, the claim follows.
      \end{proofclaim}

      \begin{clm}
        \label{proof-lb1:clm2}
        For every $i \in [1,q]$, if $C_i \cup N_i \neq \emptyset$ then the rule applied to $\separ{A_i,B_i}$ in $\Tree$ is either~\ruleFuture or~\ruleGlobally.
      \end{clm}

      \begin{proofclaim}
        By definition of $\Tree'$, the only rules that can be applied to $\separ{A_i,B_i}$ are~\ruleAtomic,~\ruleFuture and~\ruleGlobally. Suppose  $C_i \cup N_i \neq \emptyset$. We consider two cases, depending on the non-emptiness of $C_i$ and $N_i$. 
        \begin{itemize}
          \item If there is a pair $(a,b) \in C_i$, then $a \approx b$ and $(a,b) \in A_i \times B_i$.
          By definition of $\approx$, $a[0] = b[0]$, and so the rule~\ruleAtomic cannot be applied to $\separ{A_i,B_i}$.
          \item If there is $(a,b) \in N_i$ then, by \Cref{proof-lb1:clm1}, ${a,b \in (\emptyset^{v} \cdot (2^Q)^*)}$ for some $v \geq 1$.
          Hence $a[0] = b[0]$, so the rule~\ruleAtomic cannot be applied to $\separ{A_i,B_i}$.
        \end{itemize}
        Since $C_i \cup N_i \neq \emptyset$, from the two cases above we conclude that only 
        the rules~\ruleFuture and~\ruleGlobally can be 
        applied to $\separ{A_i,B_i}$.
      \end{proofclaim}

      \begin{clm}
        \label{proof-lb1:clm3}
        For every $i \in [1,q]$, $\abs{N_i} \leq 1$.
      \end{clm}
      \begin{proofclaim}
        \emph{Ad absurdum}, suppose $\abs{N_i} \geq 2$. Pick distinct $(a_1,b_1),(a_2,b_2) \in N_i$. 
        From~\Cref{proof-lb1:clm1}, the following equations hold:
        \begin{center}
          \mbox{
          $\begin{aligned}
            a_1' &\ =\ \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)-v} \cdot a_1,\\
            b_1' &\ =\ \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)-v} \cdot b_1,\\ 
            b_1'    &\ =\ (\Enum|_{-\rho_{k}})\sffx{r_{k}},\\
            a_1  &\ =\ \emptyset^{v} \cdot \rho_{k} \cdot \emptyset^{\alpha(n)-v} \cdot b_1,\\
            b_1 &\ =\ \emptyset^{v} \cdot \sigma,
          \end{aligned}$
          \qquad
          $\begin{aligned}
            a_2' &\ =\ \emptyset^{u'} \cdot \rho' \cdot \emptyset^{\alpha(n)-v'} \cdot a_2,\\
            b_2' &\ =\ \emptyset^{u'} \cdot \rho' \cdot \emptyset^{\alpha(n)-v'} \cdot b_2,\\
            b_2' &\ =\ (\Enum|_{-\rho_{\ell}})\sffx{r_{\ell}},\\
            a_2  &\ =\ \emptyset^{v'} \cdot \rho_{\ell} \cdot \emptyset^{\alpha(n)-v'} \cdot b_2,\\
            b_2 &\ =\ \emptyset^{v'} \cdot \mu,
          \end{aligned}$
          }
        \end{center}
        for some $(a_1',b_1'), (a_2',b_2') \in A \times B$, 
        $u,v,u',v' \in \N$, $k,\ell \in [1,m]$, $\rho,\rho' \in T_Q$ and $\sigma,\mu \sqsubseteq \Enum$. Moreover, $\xi_i = u+1+\alpha(n)-v = u'+1+\alpha(n)-v'$, 
        and so   
        $u-v = u'-v'$.
        By definition of $A$ and $A_i$, and from the equations above, we conclude that $a_1,a_2,b_1,b_2$ are suffixes of $\Enum$, and that $b_1 \sqsubseteq a_1$ and $b_2 \sqsubseteq a_2$. 
        From~\Cref{lemma:future-globally-disabled} and~\Cref{proof-lb1:clm2} we conclude that $a_2 \not\sqsubseteq b_1$ and $a_1 \not\sqsubseteq b_2$. 
        Therefore, $b_1 \sqsubseteq a_2$ and $b_2 \sqsubseteq a_1$.
        Since $a_1'$ and $a_2'$ are suffixes of $\Enum$, 
        we have $a_1' \sqsubseteq a_2'$ or $a_2' \sqsubseteq a_1'$. 
        Below, we consider the case $a_1' \sqsubseteq a_2'$; the other case is analogous. We split the proof into three cases, 
        each yielding a contradiction and thus resulting in $\abs{N_i} \leq 1$.
        
        \textit{Case 1: $\rho = \rho'$.} 
          From the equations above, we have 
          \begin{align*}
            a_1' \ =\ \emptyset^{u} \cdot &\rho \cdot \emptyset^{\alpha(n)} \cdot \rho_k \cdot \emptyset^{\alpha(n)-v} \cdot b_1,\\
            a_2' \ =\ \emptyset^{u'} \cdot &\rho \cdot \emptyset^{\alpha(n)} \cdot \rho_\ell \cdot \emptyset^{\alpha(n)-v'} \cdot b_2,
          \end{align*}
          By definition of $\Enum$ we get $\rho_k =
          \rho_\ell$ and so $k = \ell$ by definition of $B$.
          Together with $b_1' =
          (\Enum|_{-\rho_{k}})\sffx{r_{k}}$ and $b_2' =
          (\Enum|_{-\rho_{\ell}})\sffx{r_{\ell}}$, this implies
          $b_1' = b_2'$. Since $a_1' \approx b_1'$ and $a_2'
          \approx b_2'$, by definition of $A$ we then get
          $a_1' = a_2'$. Hence $u=u'$ and $v=v'$, and we
          conclude that $a_1 = a_2$ and $b_1 = b_2$. This
          contradicts $(a_1,b_1) \neq (a_2,b_2)$; and thus
          $\abs{N_i} \leq 1.$

        \textit{Case 2: $\rho$ is the successor of $\rho'$ in the strict total order $\prec$ used to define $\Enum$.} By definition of $\Enum$ and from the equations above, $\rho = \rho_\ell$.
          Then, we have: 
          \begin{align*}
            a_2' \ =\ \emptyset^{u'} \cdot \rho' \cdot \emptyset^{\alpha(n)} \cdot &\rho \cdot \emptyset^{\alpha(n)} \cdot \mu,\\
            a_1' \ =\ \emptyset^{u} \cdot &\rho \cdot \emptyset^{\alpha(n)} \cdot \rho_k \cdot \emptyset^{\alpha(n)-v} \cdot b_1.
          \end{align*}
          Since $a_1' \sqsubseteq a_2' \sqsubseteq \Enum$, 
          we conclude that $\mu = \rho_k \cdot \emptyset^{\alpha(n)-v} \cdot b_1$. 
          Therefore, $a_1 = \emptyset^v \cdot \mu$ and $b_1 = \emptyset^{v'} \cdot \mu$. 
          By~\Cref{lemma:prefix-length-proof,lemma:weakening-sets}, 
          the minimal deduction tree for $\separ{A_i,B_i}$ 
          has size $\min(v,v')+1 = \min(v,u'+v-u)+1$.
          Since the number of rules~\ruleNext and~\ruleWeakNext in the path of $\Tree$ from $\separ{A,B}$ to $\separ{A_i,B_i}$ is $\xi_i = u+1+\alpha(n)-v$, we conclude that 
          \begin{align*} 
            s &\geq u+1+\alpha(n)-v + \min(v,u'+v-u)+1\\
              &\geq \alpha(n) + 2 + \min(u,u').
          \end{align*}
          However, this contradicts the hypothesis $s \leq \alpha(n)$. Hence, $\abs{N_i} \leq 1$.
        
        \textit{Case 3: $\rho$ is neither equal nor the successor of $\rho'$.} Since we are assuming $a_1' \sqsubseteq a_2'$, from the equations above and the definition of $\Enum$ we conclude that $\rho$ occurs in $\mu$. More precisely, $\rho \cdot \emptyset^{\alpha(n)-v} \cdot a_1$ is a suffix of $\mu$, which implies
          that $a_1$ is a strict suffix of $b_2$.
          This contradicts $b_2 \sqsubseteq a_1$. 
          Hence, $\abs{N_1} \leq 1$.
      \end{proofclaim}

      \begin{clm}
        \label{proof-lb1:clm4}
        $\abs{C} \leq \sum_{i=1}^q \abs{C_i \cup N_i}$.
      \end{clm}
      \begin{proofclaim}
        The claim follows as soon as we prove the following 
        two statements: 
        \begin{enumerate}
          \item\label{clm4-it1} for every $(a,b) \in C$ there is $i \in [1,q]$ such that $(a\sffx{\xi_i},b\sffx{\xi_i}) \in C_{i} \cup N_i$,
          \item\label{clm4-it2} for all distinct $(a_1,b_1),(a_2,b_2) \in C$, we have $(a_1\sffx{\ell},b_1\sffx{\ell}) \neq (a_2\sffx{\ell},b_2\sffx{\ell})$ for every 
          $\ell \leq \alpha(n)$ (recall that $\xi_i \leq \alpha(n)$, for every $i \in [1,q]$).
        \end{enumerate}
        
        Let us prove~\Cref{clm4-it1}.
        By~\Cref{lemma:all-pairs-are-considered}, 
        for every $(a,b) \in C$ there is $i \in [1,q]$ 
        such that ${(a\sffx{\xi_i},b\sffx{\xi_i}) \in A_i \times B_i}$. By definition of $C_i$ and $N_i$, 
        if $a\sffx{\xi_i} \approx b\sffx{\xi_i}$ 
        then $(a\sffx{\xi_i},b\sffx{\xi_i}) \in C_i$, 
        and otherwise $(a\sffx{\xi_i},b\sffx{\xi_i}) \in N_i$.
        
        We move to~\Cref{clm4-it2}. Since $(a_1,b_1)$
        and $(a_2,b_2)$ belong to $C$, we have $a_1 \approx
        b_1$ and $a_2 \approx b_2$. By definition of
        $\approx$ and~$\Enum$, this means that the length of
        the traces $a_1,a_2,b_1,b_2$ is at least
        $\alpha(n)+1$. 
        
        Suppose first that $a_1 \neq a_2$. 
        Then, from the fact that
        $a_1,a_2 \sqsubseteq \Enum$ we conclude that
        $a_1\sffx{\ell} \neq a_2\sffx{\ell}$ for all $\ell
        \leq \alpha(n)$, and thus
        $(a_1\sffx{\ell},b_1\sffx{\ell}) \neq
        (a_2\sffx{\ell},b_2\sffx{\ell})$. 

        Consider now the case $a_1 = a_2$, and so $b_1 \neq b_2$. In this case, from  $a_1 \approx
        b_1$ and $a_2 \approx b_2$, we derive $b_1 \approx
        b_2$, and so there are $u \in \N$, $\rho \in T_Q$ 
        and $\sigma_1,\sigma_2 \in (2^Q)^*$ 
        such that 
        $b_1 = \emptyset^u \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma_1$ 
        and 
        $b_2 = \emptyset^u \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma_2$. 
        From $b_1 \neq b_2$, it follows that $\sigma_1 \neq \sigma_2$. Let $\ell \in [0,\alpha(n)]$. 
        Clearly $\sigma_1 \sqsubseteq b_1\sffx{\ell}$ 
        and $\sigma_2 \sqsubseteq b_2\sffx{\ell}$, 
        and therefore $b_1\sffx{\ell} \neq b_2\sffx{\ell}$.
        Then, $(a_1\sffx{\ell},b_1\sffx{\ell}) \neq
        (a_2\sffx{\ell},b_2\sffx{\ell})$.
      \end{proofclaim}

      \vspace{5pt}
      We are now ready to prove that $s \geq \abs{C}+1$, concluding the proof for~\ruleNext and~\ruleWeakNext: 
      \begin{align*}
        s &\geq 1 + \sum_{i=1}^q s_i 
          &\text{by definition~of $\Tree$ and $\Tree'$}\\
          &\geq 1+\sum_{i=1}^q (\abs{C_i}+1) 
          &\text{by $s_i \geq \abs{C_i}+1$ (induction hypothesis)}\\
          &\geq 1+\sum_{i=1}^q (\abs{C_i \cup N_i})
          &\text{by $\abs{N_i} \leq 1$ (\Cref{proof-lb1:clm3})}\\
          &\geq \abs{C}+1
          &\text{by $\textstyle\abs{C} \leq \sum_{i=1}^q \abs{C_i \cup N_i}$ (\Cref{proof-lb1:clm4}).}
      \end{align*}


      
    \item[\textbf{case: rule~{\rm{\ruleFuture}}.}]
      Let $f \in \FP_A$ be the future point used when applying this rule. The minimal
      deduction tree for $\separ{A^f,B^{\ltl{G}}}$ has size
      $s-1$. Let $a \in A^f$ be such that for every $a'' \in A^f$, $a \sqsubseteq a''$. The existence of such an element $a$ is guaranteed from the fact that all elements in $A$ and $A^f$ are suffixes of~$\Enum$.
      We define $C' \coloneqq \{(a',b') \in A^f \times B^{\ltl{G}} : a' \approx b' \}$ and $C_a \coloneqq \{b \in B^{\ltl{G}} : a \approx b\}$. By induction hypothesis, $s-1 \geq \abs{C'} + 1$, i.e., $s \geq \abs{C'} + 2$. 
      Since $\abs{C'} \geq \abs{C_a}$, we have $s \geq \abs{C_a}+2$ and to conclude the proof it suffices to show that $\abs{C_a} \geq \abs{C}-1$.
      We do so by establishing a series of claims.
      Below, recall that we are assuming $\abs{C} \geq 2$.
      \begin{clm}
        \label{proof-lbF-clm1}
        For every $b \in B^{\ltl{G}}$, $a \not\sqsubseteq b$.
      \end{clm}
      \begin{proofclaim}
        \emph{Ad absurdum} 
        suppose there is $b \in B^{\ltl{G}}$ such that $a \sqsubseteq b$. Then, by definition of $B^{\ltl{G}}$ we conclude that $a \in B^{\ltl{G}}$.
        However, this contradicts the existence of $\Tree$ by~\Cref{lemma:unclosable-tree-condition} and~\Cref{th:ps}.
      \end{proofclaim}

      \begin{clm}
        \label{proof-lbF-clm2}
        There are $u \in \N$ $\rho \in T_Q$ and $\sigma \in (2^{Q})^*$ such that $a = \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$.
      \end{clm}
      \begin{proofclaim}
        Since $a$ is a suffix of $\Enum$, 
        we either have $a = \emptyset^v$ for some $v \in [1,\alpha(n)]$, or there are $u \in \N$ $\rho \in T_Q$ and $\sigma \in (2^{Q})^*$ such that $a = \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$.
        The former case is however impossible in our setting:
        since $\abs{C} \geq 2$, by definition of $\approx$ and $B$, the former case implies that there is $b \in B$ having $\emptyset^{\alpha(n)}$ as a suffix. 
        Then $a = \emptyset^v \in B^{\ltl{G}}$, 
        contradicting~\Cref{proof-lbF-clm1}.
      \end{proofclaim}

      \vspace{5pt}
      Below, we write $u,\rho$ and $\sigma$ for the objects 
      appearing in~\Cref{proof-lbF-clm2}. 
      Recall that $\prec$ denotes the order used to define $\Enum$.
      
      \begin{clm}
        \label{proof-lbF-clm3}
        For every $(a',b') \in C$ and $k \in [1,q]$ with $b' = (\Enum|_{\rho_k})\sffx{r_k}$, 
        $\rho \preceq \rho_k$.
      \end{clm}
      \begin{proofclaim}
        \emph{Ad absurdum}, suppose there is $(a',b') \in C$ and $k \in [1,q]$ such that $b' = (\Enum|_{\rho_k})\sffx{r_k}$ and $\rho_k \prec \rho$.
        Since $(a',b') \in C$, there are $v \in \N$, $\rho' \in T_Q$ and $\sigma_1,\sigma_2 \in (2^{Q})^*$ such that 
        $a' = \emptyset^v \cdot \rho' \cdot \emptyset^{\alpha(n)} \cdot \sigma_1$ and 
        $b' = \emptyset^v \cdot \rho' \cdot \emptyset^{\alpha(n)} \cdot \sigma_2$.
        From~\Cref{claim-rho-prec-rhok}, $\rho' \prec \rho_k$. 
        Again by definition of $\Enum|_{-\rho_k}$ and from $\rho_k \prec \rho$, 
        we conclude that one of the suffixes of $b'$ is the suffix of $\Enum$ having the form $\emptyset^{\alpha(n)} \cdot \rho \cdot \sigma'$, for some $\sigma' \in (2^Q)^*$. Then, $a \sqsubseteq b'$. 
        However, since $b' \in B^{\ltl{G}}$, this contradicts~\Cref{proof-lbF-clm1}. Hence, $\rho \preceq \rho_k$.
      \end{proofclaim}

      \vspace{5pt}
      Let $I \subseteq [1,m]$ be the subset of those indices $i \in [1,m]$ such that $(\Enum|_{\rho_i})\sffx{r_i}$ 
      appears in the second component of a pair in~$C$, 
      i.e., there is $(a',b') \in C$ such that $b' = (\Enum|_{\rho_i})\sffx{r_i}$. Suppose $I = \{i_1,\dots,i_q\}$,
      and without loss of generality assume $\rho_{i_1} \prec \rho_{i_2} \prec \dots \prec \rho_{i_q}$.
      Note that, 
      given $(a',b'),(a'',b') \in C$ 
      we have $a' = a''$,
      by definition of $\approx$, $A$ and $C$.
      Therefore, $q = \abs{C}$.
      By~\Cref{proof-lbF-clm3}, ${\rho \prec \rho_{i_2} \prec \dots \prec \rho_{i_q}}$.      
      For $i \in I \setminus \{i_1\}$, 
      consider $(a_i',b_i') \in C$ with $b_i' \coloneqq (\Enum|_{\rho_i})\sffx{r_i}$.

      \begin{clm}
        \label{proof-lbF-clm4}
        For each $i \in I \setminus \{i_1\}$ there is $\ell \in \N$
        such that $a \approx b_i''$ with $b_i'' \coloneqq b_i'\sffx{\ell}$.
        Moreover, $b_i''$ contains all types in $\{\rho_{i_2}, \dots, \rho_{i_q}\}$, except for $\rho_i$. 
      \end{clm}

      \begin{proofclaim}
        By~\Cref{claim-rho-prec-rhok},
        there are $v \in \N$, $\rho' \in T_Q$ and $\sigma' \in (2^Q)^*$
        such that $\rho' \prec \rho_i$ and $b_i' = \emptyset^{v} \cdot \rho' \cdot \emptyset^{\alpha(n)} \cdot \sigma'$.
        Since $a \sqsubseteq a''$ for every $a'' \in A^f$, 
        by definition of $f$ we get $a \sqsubseteq a'$.
        Since $a' \sqsubseteq \Enum$, we derive $\rho' \preceq \rho \prec \rho_i$. This implies that there is a suffix~$b_i''$ of $b_i'$ 
        of the form $\emptyset^u \cdot \rho \cdot \emptyset^\alpha(n) \cdot \sigma''$.
        By~\Cref{proof-lbF-clm2},~$a \approx b_i''$.
        From $\rho \prec \rho_{i_2} \prec \dots \prec \rho_{i_q}$ and by definition of~$\Enum|_{\rho_i}$, 
        we conclude that $b_i''$ contains all types in $\{\rho_{i_2}, \dots, \rho_{i_q}\}$, except for $\rho_i$.
      \end{proofclaim}

      \vspace{5pt}
      Following up on the second statement in~\Cref{proof-lbF-clm4}, 
      since all types $\rho_{i_2}, \dots, \rho_{i_q}$ are distinct, 
      we conclude that $b_i'' \neq b_j''$ for every two distinct $i,j \in I \setminus \{i_1\}$.
      Then, the first statement in~\Cref{proof-lbF-clm4}
      entails $\abs{C_a} \geq q-1 = \abs{C}-1$. 
      This concludes the proof of the case~\ruleFuture.

      

    \item[\textbf{case: rule~{\rm{\ruleGlobally}}.}] 
      Let $f \in \FP_A$ be the future point used when applied this rule. The minimal deduction tree for $\separ{A^{\ltl{G}},B^f}$ has size $s-1$. 
      Let $a \in A$ such that $a'' \sqsubseteq a$ for every $a'' \in A$. The existence of such an element $a$ is guaranteed from the fact that all elements in $A$ are suffixes of~$\Enum$. 
      Note that~$a$ and all its suffixes belong to $A^{\ltl{G}}$.
      We define ${C' \coloneqq \{(a',b') \in A^{\ltl{G}} \times B^{f} : a' \approx b' \}}$. By induction hypothesis, $s-1 \geq \abs{C'} + 1$, i.e., $s \geq \abs{C'} + 2$. To conclude the proof it suffices to show that $\abs{C'} \geq \abs{C}-1$ (in fact, we prove~$\abs{C'} \geq \abs{C}$).
      Let $\{(a_1,b_1),\dots,(a_{\abs{C}},b_{\abs{C}})\} = C$.

      \begin{clm}
        \label{proof-lbG-clm1}
        For every $i \in [1,\abs{C}]$, 
        $b_i^f$ is not a suffix of $\Enum$. 
        More precisely, given $k \in [1,m]$ such that $b_i = (\Enum|_{-\rho_k})\sffx{r_k}$, 
        there are $u \in \N$, $\rho \in T_Q$ and $\sigma$ 
        such that $b_i^f = \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$ and $\rho \prec \rho_k$.
      \end{clm}

      \begin{proofclaim}
        Note that the second statement is implied by the first one, directly from the definition of~$\Enum|_{-\rho_k}$ and since $b_i \in B$.
        For the first statement,
        \emph{ad absurdum}, suppose that $b_i^f$ is a suffix of $\Enum$.
        By definition of $\Enum$ and since $a_i \approx b_i$,
        we have $b_i^f \sqsubseteq a_i$.
        From $a_i \sqsubseteq a$ we then conclude $b_i^f \in A^{\ltl{G}}$. However, this contradicts the existence of $\Tree$ by~\Cref{lemma:unclosable-tree-condition} and~\Cref{th:ps}. Hence, $b_i^f$ is not a suffix of $\Enum$. 
      \end{proofclaim}

      \begin{clm}
        \label{proof-lbG-clm2}
        For every $i \neq j \in [1,\abs{C}]$, $b_i^f \neq b_j^f$.
      \end{clm}

      \begin{proofclaim}
        \emph{Ad absurdum}, suppose $b_i^f = b_j^f$. 
        By definition of $B$, $b_i = (\Enum|_{-\rho_{k_1}})\sffx{r_{k_1}}$ and 
        $b_j = (\Enum|_{-\rho_{k_2}})\sffx{r_{k_2}}$ 
        for some $k_1 \neq k_2 \in [1,m]$.
        We have $\rho_{k_1} \neq \rho_{k_2}$.
        Then, $b_i^f = b_j^f$ 
        implies $b_i^f \sqsubseteq \Enum$. 
        However, this contradicts~\Cref{proof-lbG-clm1}. 
        So, $b_i^f \neq b_j^f$.
      \end{proofclaim}

      \begin{clm}
        \label{proof-lbG-clm3}
        For every $i \in [1,\abs{C}]$ there is $\ell \in \N$ 
        such that $a\sffx{\ell} \approx b_i^f$.
      \end{clm}

      \begin{proofclaim}
        Following~\Cref{proof-lbG-clm1}, there are $u \in \N$, $\rho \in T_Q$ and $\sigma \in (2^Q)^*$ 
        such that $b_i^f = \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma$.
        By definition of $\Enum$ and since $a_i \sqsubseteq a$, 
        every element of $T_Q$ appearing in $b_i$ also appears in $a$. Then, there is $\ell \in \N$ and $\sigma' \in (2^Q)^*$ such that $a\sffx{\ell} = \emptyset^{u} \cdot \rho \cdot \emptyset^{\alpha(n)} \cdot \sigma'$.
        Therefore, $a\sffx{\ell} \approx b_i^f$.
      \end{proofclaim}

      \vspace{5pt}
      Together,~\Cref{proof-lbG-clm2,proof-lbG-clm3}
      directly imply $\abs{C'} \geq \abs{C}$.
      This concludes both the proof of the case~\ruleGlobally 
      and the proof of the lemma.
      \qedhere
  \end{itemize}
\end{proof}

%%% INFINITE CASE

% \begin{lemma} \label{lemma:lower-bound:spoon-case}
%   Consider $j,k_1,\dots,k_n \in \N$ as well as distinct
%   sets ${\rho_1,\dots,\rho_n \in T_Q}$, for some $n \in
%   \N$. Let $a \coloneqq (\Enum)^\omega$, $A \coloneqq \{
%   (a, j) \}$ and $B \coloneqq
%   \{\left(\left(\Enum|_{-\rho_i}\right)^\omega, k_i
%   \right) : i \in [1,n] \}$. Let $m$ be the number of
%   $(w,i) \in B$ such that $w[i] = a[j]$. The minimal
%   deduction tree of $(A,B)$ has size at least $m$.
%   \end{lemma}

% \am{I think that $m$ above is essentially a sub-additive
% proof measure defined on a subset of all models.}

% \begin{proof} We prove the statement by induction on the
%   size of the minimal deduction tree. Let~$\Tree$ be a
%   minimal deduction tree for $(A,B)$, and suppose it has
%   size $k$. \begin{description} \item[base case $k = 1$.]
%   In this case, $\Tree$ is a simple application of the
%   rule~\ruleAtomic. Then, there must be $q \in Q$ such
%   that either $q \in a[j]$ and $q \not \in w[i]$ for every
%   $(w,i) \in B$, or vice versa, i.e.,  $q \not \in a[j]$
%   and $q \in w[i]$ for every $(w,i) \in B$. We conclude
%   that every $(w,i) \in B$ is such that $w[i] \neq a[j]$,
%   and thus $m = 0$ and the statement is proven.
%   \item[induction step $k \geq 2$.] Note that if $m = 0$
%   or $m = 1$ then the statement is trivially satisifed. So
%   let us assume~$m \geq 2$. We split the proof depending
%   on the rule applied to the root $(A,B)$ of $\Tree$. Note
%   that this rule cannot be~\ruleAtomic, since $k \geq 2$.
%   \begin{description} \item[rule~\ruleOr.] In this case
%   given $A_1,A_2$ such that $A_1 \uplus A_2 = A$ we have
%   either $A_1 = A$ or $A_2 = A$. This contradicts the
%   minimality of $\Tree$, hence showing that the root of
%   $\Tree$ is not an \ruleOr rule. \item[rule \ruleAnd.]
%   Consider $B_1,B_2$ such that $B_1 \uplus B_2 = B$. Note
%   that $|B_1| + |B_2| = |B| = n$. Given $\ell \in \{1,2\}$
%   let $m_\ell$ be the number of $(w,i) \in B_\ell$ such
%   that $w[i] = a[j]$, and let $k_\ell$ be the size of the
%   minimal deduction tree of $(A,B_\ell)$. By definition
%   of $B_1$ and $B_2$, $m = m_1 + m_2$ and $k = k_1 + k_2 +
%   1$. By induction hypothesis, $m_1 \leq k_1$ and $m_2
%   \leq k_2$, hence $m \leq k_1 + k_2 < k$. \item[rule
%   \ruleNext.] the minimal deduction tree for
%   $(A^{\ltl{X}},B^{\ltl{X}})$ has size $k-1$. To conclude
%   that $\Tree$ has size $m$ it suffices to show that the
%   minimal deduction tree for $(A^{\ltl{X}},B^{\ltl{X}})$
%   has size at least $m-1$. Let $(w_1,i_1),\dots,(w_m,i_m)$
%   be the $m$ elements of $B$ such that $w_\ell[i_\ell] =
%   a[j]$ for all $\ell \in [1,m]$. By definition, $a[j+1]$
%   is the successor of $a[j]$ in the enumeration $\Enum$
%   (where the successor of the last element in $\Enum$ is
%   its first element). \emph{Ad absurdum}, suppose that
%   there are two distinct $\ell,r \in [1,m]$ such that
%   $w_\ell[i_\ell+1] \neq a[j+1]$ and $w_r[i_r+1] \neq
%   a[j+1]$. By definition of $B$ and of
%   $(\Enum|_{-\rho_i})$, we conclude that $w_\ell = w_r =
%   (\Enum|_{-\rho_i})^\omega$ for some $i \in [1,n]$.
%   However, each element of $B$ is of the form
%   $\left(\left(\Enum|_{-\rho}\right)^\omega, k \right)$
%   for a distinct $\rho \in T_Q$; a contradiction. We
%   conclude that at most one among
%   $(w_1,i_1+1),\dots,(w_m,i_m+1)$ can be distinct from
%   $a[j+1]$. By definition of $(A^{\ltl{X}},B^{\ltl{X}})$
%   and by induction hypothesis, this means that the minimal
%   deduction tree for $(A^{\ltl{X}},B^{\ltl{X}})$ has size
%   at least $m-1$. \item[rule \ruleFuture.] Let $\sigma \in
%   \Sigma_A$ be the future point used in this rule.
%   Similarly to the previous case, to conclude the proof it
%   suffices to show that the minimal deduction tree for
%   $(\sigma(A),B^{\ltl{F}})$ has size at least $m-1$. In
%   fact, we show that this tree has size at least $n-1$.
%   Note that by definition $m \leq n$. By definition,
%   $\sigma(A) = \{(a,\sigma(a,j))\}$. Let $\rho \coloneqq
%   a[\sigma(a,j)]$. By definition of $B$, there is at most
%   one $(w,i) \in B$ such that $w =
%   (\Enum|_{-\rho})^\omega$, meaning that $\rho$ appears in
%   at least $n-1$ words in $B$. Therefore, $B^{\ltl{F}}$
%   contains at least $n-1$ pairs $(w',i')$ such that
%   $w'[i'] = \rho$. Let $B'$ be a set of $n-1$ such pairs.
%   Since $(\sigma(A),B^{\ltl{F}})$ has a deduction tree of
%   size $k-1$, and $B' \subseteq B^{\ltl{F}}$, we conclude
%   that $(\sigma(A),B')$ has a deduction tree of size at
%   most $k-1$. By induction hypothesis, the minimal
%   deduction tree for $(\sigma(A),B')$ has size at least
%   $n-1$, and therefore the same holds true for
%   $(\sigma(A),B^{\ltl{F}})$,
%   by~\Cref{lemma:weakening-sets}. \qedhere
%   \end{description} \end{description} \end{proof}

% \begin{lemma} \label{lemma:lower-bound:one-more-step} Let
%   $j \in \N$. Consider distinct sets ${\rho_1,\dots,\rho_n
%   \in T_Q}$, for some $n \in \N$. Let $a \coloneqq
%   \emptyset^{j} \cdot (\Enum)^\omega$, $A \coloneqq \{ (a,
%   0) \}$ and $B \coloneqq \{\left( \emptyset^{j} \cdot
%      \left(\Enum|_{-\rho_i}\right)^\omega,\, 0 \right) : i
%      \in [1,n] \}$. The minimal deduction tree of $(A,B)$
%      has size at least $n-1$. \end{lemma}

% \begin{proof} Let $\Tree$ be the minimal deduction tree
% of $(A,B)$, assumed to have size $k$.  
% The proof is by induction on $(j,k)$ with respect to the
% lexicographic order. \begin{description} \item[base case
% $j = 0$.] In this case, $A$ and $B$ are sets of traces
% considered in~\Cref{lemma:lower-bound:spoon-case}. Since
% $\rho_1,\dots,\rho_n$ are distinct, there are at least
% $n-1$ pairs $(w,0) \in B$ such that $w[0] = a[0]$. Then,
% $\Tree$ has size at least $n-1$, directly
% from~\Cref{lemma:lower-bound:spoon-case}. \item[base case
% $k = 1$.] In this case, $\Tree$ is a simple application of
% the rule~\ruleAtomic. Note that then $j$ must be $0$,
% since otherwise all traces in $A \cup B$ would start with
% $\emptyset$ and~\ruleAtomic cannot be used. Then, the
% proof follows as in the previous case. \item[induction
% case $j \geq 1$ and $k \geq 2$.] Note that the
% rule~\ruleAtomic cannot be applied, since all traces in $A
% \cup B$ start with $\emptyset$. We split the proof
% depending on the rule applied to the root of $\Tree$.
% \begin{description} \item[rule~\ruleOr.] In this case
% given $A_1,A_2$ such that $A_1 \uplus A_2 = A$ we have
% either $A_1 = A$ or $A_2 = A$. This contradicts the
% minimality of $\Tree$, hence showing that the root of
% $\Tree$ is not an \ruleOr rule. \item[rule \ruleAnd.]
% Consider $B_1,B_2$ such that $B_1 \uplus B_2 = B$. Note
% that $|B_1| + |B_2| = |B| = n$. Since $\Tree$ is the
% minimal deduction tree of $(A,B)$, the minimal deduction
% trees of $(A,B_1)$ and $(A,B_2)$ have sizes $k_1$ and
% $k_2$ respectively, with $k_1+k_2+1 = k$. By induction
% hypothesis, $k_1 \leq |B_1|-1$ and $k_2 \leq |B_2|-1$.
% Therefore, $k \leq |B_1|+|B_2|-1 = n-1$. \item[rule
% \ruleNext.] The statement holds directly by induction
% hypothesis. \item[rule \ruleFuture.] Let $\sigma \in
% \Sigma_A$ be the future point used in this rule. Note that
% we cannot have $\sigma((a,0)) = 0$, else we reach a
% contradiction with the minimality of $\Tree$. If
% $\sigma((a,0)) \in [1,j-1]$, then $(a,\sigma(a,0))$ is of
% the form $\emptyset^{j'} \cdot (\Enum)^\omega$ with $j' <
% j$ and the statement follows by induction hypothesis. If
% instead $\sigma((a,0)) \geq j$, from the fact that
% $\rho_1,\dots,\rho_n$ are distinct we conclude that there
% is a set $B' \subseteq B^{\ltl{F}}$ of $n-1$ traces such
% that $w[\ell] = a[\sigma(a,0)]$ for every $(w,\ell) \in
% B'$. The statement then follows
% by~\Cref{lemma:lower-bound:spoon-case}. \qedhere
% \end{description} \end{description} \end{proof}

==> sections/proof-system-until.tex <==
%! root=../main.tex

\section{A proof system for $\mathsf{coSafety{\text-}LTL}$}
\label{sec:psuntil}

Given $f \in \FP_A$, we define $(f,A)^{\forall} \coloneqq \set{(\sigma,j)
\suchthat (\sigma,i) \in A,\, i \leq j < f(\sigma,i)}$. 
We define $\Pi_B \coloneqq \set{(\sigma,i,j) \suchthat (\sigma,i) \in
B , (\sigma,j) \in B^{\ltl{F}}}$.
Given two subsets $B_1,B_2 \subseteq B^{\ltl{F}}$, we say that the pair
$(B_1,B_2)$ is \emph{until-complete for $\Pi_B$} iff, for all $(\sigma,i,j)
\in \Pi_B$, either $(\sigma,j) \in B_2$ or $(\sigma,k) \in B_1$ for some $i
\le k < j$.

\begin{mathpar} 
  \inferrule[\ruleUntil]{
    ((f,A)^{\forall},B_1) 
      \and
    (f(A),B_2) 
      \and 
    f\in\FP_A 
      \and
    B_1,B_2 \subseteq B^{\ltl{F}}
      \and
    (B_1,B_2) \text{ until-complete for } \Pi_B 
  }
  { (A,B) }
\end{mathpar}

In the setting of Adler-Immerman games, the \ruleUntil rule corresponds to
the following moves of Spoiler and Duplicator. First, for each $(\sigma,i)
\in A$, Spoiler chooses an interval of $\sigma$ starting from $i$, with the
intention of having this interval satisfying a formula of the type
$\ltl{\Phi_1 U \Phi_2}$. Duplicator plays optimally in $B$ by moving to all
possible future time points of $(\sigma,i)$, for each $(\sigma,i) \in B$.
Second, two nodes of the game tree $(A_1,B_1)$ and $(A_2,B_2)$ are created
in the following way. Spoiler now plays in $B$ and he partition the
intervals choosen by Duplicator into two sets: for each path $\sigma$ in
the first set, Spoiler chooses a point $j$ in the interval different from
the last one and places $(\sigma,j)$ in $B_1$; conversely, for each path
$\sigma$ in the second set, Spoiler places its last time point $(\sigma,k)$
in $B_2$.  For each interval choosen by Spoiler in the first part of the
move, Duplicator places \emph{all} its points except from the last one in
$A_1$ and \emph{all} its last points in $A_2$.

\begin{theorem}
\label{th:psu}
  The pair $(A,B)$ has a derivation tree of size $k$ if and only if there
  is a formula~$\Phi$ of \cosafetyltl of size $k$ such that $A \models
  \Phi$ and $B \pperp \Phi$.
\end{theorem}
\begin{proof}
  We only consider the inductive case for the \ruleUntil rule, since the
  base case and the other inductive cases are the same of \cref{th:ps}.

  $(\Rightarrow)$
  Given a derivation tree for $(A,B)$ of size $k$, we build a \cosafetyltl
  formula $\Phi$ of size $k$ such that $A\models \Phi$ and $B \pperp \Phi$.

  \begin{description}
    \item[rule \ruleUntil.] Let $((f,A)^{\forall}, B_1)$ and $(f(A), B_2)$
      be the two children of the root node.  By inductive hypothesis, there
      exist two \cosafetyltl formulae $\Phi_1$ and $\Phi_2$ such that:
      \begin{itemize}
        \item $(f,A)^{\forall} \models \Phi_1$ and $B_1 \pperp \Phi_1$; and
        \item $f(A) \models \Phi_2$ and $B_2 \pperp \Phi_2$.
      \end{itemize}

      We show that $A \models \ltl{\Phi_1 U \Phi_2}$. Let $(\sigma,i) \in
      A$ and let $j = f(\sigma,i)$. Since $(\sigma,j) \in f(A)$, it holds
      that $(\sigma,j) \models \Phi_2$. Moreover, by construction of
      $(f,A)^{\forall}$, we have that $(\sigma,k) \in (f,A)^{\forall}$, for
      any $k<j$, and thus $(\sigma,k) \models \Phi_1$, for any $k<j$.
      Therefore, $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$.

      Now we prove that $B \pperp \ltl{\Phi_1 U \Phi_2}$. Suppose by
      contradiction that there exists a pair $(\sigma,i) \in B$ such that
      $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$. Let $j\in\N$ be such that
      $(\sigma,j) \models \Phi_2$ and $(\sigma,k) \models \Phi_1$, for all
      $i\le k < j$. Since $(\sigma,i,j)$ belongs to $\Pi_B$ and since
      $(B_1,B_2)$ is \emph{until-complete for $B^{\ltl{F}}$}, it holds that
      either $(\sigma,j) \in B_2$ or $(\sigma,k) \in B_1$ for some $i \le
      k < j$.
      We divide in cases:
      \begin{itemize}
        \item if $(\sigma,j) \in B_2$, then by inductive hypothesis
          $(\sigma,j) \not \models \Phi_2$, which is a contradiction;
        \item otherwise, $(\sigma,k) \in B_1$ for some $i\le k < j$, and by
          inductive hypothesis $(\sigma,k) \not \models \Phi_1$, which is
          a contradiction.
      \end{itemize}
      Therefore, $B \pperp \ltl{\Phi U \Phi_2}$.

      It follows that $\ltl{\Phi_1 U \Phi_2}$ separates $A$ and $B$.
      Moreover, $|\ltl{\Phi_1 U \Phi_2}| = |\Phi_1| + |\Phi_2| + 1 = k$. 
  \end{description}


  $(\Leftarrow)$
  Given a formula $\Phi$ of \cosafetyltl of size $k$ such that $A \models
  \Phi$ and $B \pperp \Phi$, we build a derivation tree for $(A,B)$ of size
  $k$.

  \begin{description}
    \item[induction step: $\Phi = \ltl{\Phi_1 U \Phi_2}$.] 
      We first show that $(f,A)^{\forall} \models \Phi_1$ and $f(A) \models
      \Phi_2$ for some $f \in \FP_A$. By hypothesis, for any $a
      = (\sigma,i)$ in $A$, $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$,
      that is there exists a $j_a \ge i$ such that $(\sigma,j_a) \models
      \Phi_2$ and $(\sigma,k) \models \Phi_1$, for all $i\le k < j_a$. We
      choose $f : A \to \N$ such that $f(a) = j_a$ for any $a \in A$. With
      this choice for $f$, for all $(\sigma',j') \in f(A)$ it holds that
      $(\sigma,j') \models \Phi_2$.  Moreover, by construction of $f$ and
      of $(f,A)^{\forall}$, it holds that $(\sigma'',j'')$ for all
      $(\sigma'',j'') \in (f,A)^{\forall}$.

      Now we prove that $B_1 \pperp \Phi_1$ and $B_2 \pperp \Phi_2$ for
      some $B_1,B_2 \subseteq B^{\ltl{F}}$ such that $(B_1,B_2)$ is
      \emph{until-complete for $B^{\ltl{F}}$}.
      We define $B_1$ and $B_2$ in this way:
      \begin{itemize}
        \item $B_1 = \set{(\sigma,i) \in B^{\ltl{F}} \suchthat
          (\sigma,i) \not\models \Phi_1}$;
        \item $B_2 = \set{(\sigma,i) \in B^{\ltl{F}} \suchthat
          (\sigma,i) \not\models \Phi_2}$.
      \end{itemize}
      Clearly, $B_1 \pperp \Phi_1$ and $B_2 \pperp \Phi_2$. We prove that
      $(B_1,B_2)$ is \emph{until-complete for $B^{\ltl{F}}$}.
      %
      Since by hypothesis $B \pperp \ltl{\Phi_1 U \Phi_2}$, for all
      $(\sigma,i) \in B$ and for any $j\ge i$ it holds that:
      \begin{itemize}
        \item either $(\sigma,j) \not\models \Phi_2$;
        \item or there exists a $i\le k < j$ such that $(\sigma,k)
          \not\models \Phi_1$.
      \end{itemize}
      By construction of $B_1$ and $B_2$, it follows that for all
      $(\sigma,i,j) \in \Pi_B$, either $(\sigma,j) \in B_2$ or $(\sigma,k)
      \in B_1$ for some $i \le k < j$. Therefore, $(B_1,B_2)$ is
      \emph{until-complete for $B^{\ltl{F}}$}.

      Since $\Phi_1$ separates $(f,A)^{\forall}$ and $B_1$ and since
      $\Phi_2$ separates $f(A)$ and $B_2$, by inductive hypothesis, there
      are two derivation trees rooted at $((f,A)^{\forall},B_1)$ and
      $(f(A),B_2)$ of size $|\Phi_1|$ and $|\Phi_2|$, respectively. This
      proves that there is a derivation tree rooted at $(A,B)$ of size
      $|\Phi_1| + |\Phi_2| + 1$, that is $k$.
  \end{description}
\end{proof}

\subsection{Example}
\emph{For simplicity, instead of pairs $(\sigma,i)$ let us just keep the
suffix of the word starting at $i$.}

\begin{mathpar} 
  \inferrule*[Right = \ruleUntil]{   
    \inferrule*[Left = \ruleAtomic]{
      A \models a \and B \pperp a
    }{
      (\set{aaab,aab,ab},\set{cb})
    }
    \and
    \inferrule*[Right = \ruleAtomic]{
      A \models b \and B \pperp b
    }{
      (\set{b},\set{aaaa,aaa,aa,a,acb})
    }
  }{
    (\set{aaab},\set{aaaa,acb})
  }
\end{mathpar}

As a matter of fact, $\set{aaab} \models \ltl{a U b}$ and $\set{aaaa,acb}
\pperp \ltl{a U b}$, and the size of the above derivation tree is exactly
$|\ltl{a U b}|$.


\subsection{Alternative Version of the UNTIL rule}

For any $g \in \FP_B$, we define $g_<(B) \coloneqq
\set{(\sigma,g(\sigma,i)) \suchthat (\sigma,i) \in B , \ g(\sigma,i)
< |\sigma|-1}$ and $(g,B)^{w\forall} \coloneqq \set{(\sigma,j) \suchthat
(\sigma,i) \in B , \ i\le j \le g(\sigma,i)}$.

\begin{mathpar} 
  \inferrule[\ruleUntil]{
    ((f,A)^{\forall}, g_<(B)) 
      \and
    (f(A),(g,B)^{w\forall}) 
      \and 
    f\in\FP_A 
      \and
    g\in\FP_B 
  }
  { (A,B) }
\end{mathpar}

Intuitively, $(g,B)^{w\forall}$ and $g_<(B)$ correspond to the two
disjuncts of the semantics of $(\sigma,i) \models \ltl{(! \phi_1) R (!
\phi_2)}$ over \emph{finite traces}, that is: either $\forall i \le
j < |\sigma| \suchdot ((\sigma,j) \models \lnot \phi_2)$ or $\exists i\le
j<|\sigma| \suchdot ((\sigma,j) \models \lnot \phi_1 \land \forall i \le
k \le j \suchdot (\sigma,k) \models \lnot \phi_2)$.
In other words, if $B \pperp \ltl{\Psi_1 U \Psi_2}$ then for each
$(\sigma,i) \in B$ there always exists a position $j\ge i$ such that
$(\sigma,k) \not\models \Psi_2$ for each $i\le k \le j$ and, if
$j<|\sigma|-1$ then $(\sigma,j) \not\models \Psi_1$.
\textbf{Note:} the fact that $g_<(B)$ excludes the last position of a word
is for dealing with the case in which the word always satisfies $\Psi_1$
but never $\Psi_2$. In this case, the set $g_<(B)$ is empty.

Here below we prove the main theorem for the new version of the \ruleUntil
rule.

\begin{theorem}
\label{th:psu}
  The pair $(A,B)$ has a derivation tree of size $k$ if and only if there
  is a formula~$\Phi$ of \cosafetyltl of size $k$ such that $A \models
  \Phi$ and $B \pperp \Phi$.
\end{theorem}
\begin{proof}
  We only consider the inductive case for the \ruleUntil rule, since the
  base case and the other inductive cases are the same of \cref{th:ps}.

  $(\Rightarrow)$
  Given a derivation tree for $(A,B)$ of size $k$, we build a \cosafetyltl
  formula $\Phi$ of size $k$ such that $A\models \Phi$ and $B \pperp \Phi$.

  \begin{description}
    \item[rule \ruleUntil.] Let $((f,A)^{\forall}, g_<(B))$ and $(f(A),
      (g,B)^{w\forall})$ be the two children of the root node.  By
      inductive hypothesis, there exist two \cosafetyltl formulae $\Phi_1$
      and $\Phi_2$ such that:
      \begin{itemize}
        \item $(f,A)^{\forall} \models \Phi_1$ and $g_<(B) \pperp \Phi_1$;
          and
        \item $f(A) \models \Phi_2$ and $(g,B)^{w\forall} \pperp \Phi_2$.
      \end{itemize}

      We show that $A \models \ltl{\Phi_1 U \Phi_2}$. Let $(\sigma,i) \in
      A$ and let $j = f(\sigma,i)$. Since $(\sigma,j) \in f(A)$, it holds
      that $(\sigma,j) \models \Phi_2$. Moreover, by construction of
      $(f,A)^{\forall}$, we have that $(\sigma,k) \in (f,A)^{\forall}$, for
      any $k<j$, and thus $(\sigma,k) \models \Phi_1$, for any $k<j$.
      Therefore, $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$.

      Now we prove that $B \pperp \ltl{\Phi_1 U \Phi_2}$. Suppose by
      contradiction that there exists a pair $(\sigma,i) \in B$ such that
      $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$. Let $j\in\N$ be such that
      $(\sigma,j) \models \Phi_2$ and $(\sigma,k) \models \Phi_1$, for all
      $i\le k < j$.
      Let $g \in \FP_B$. We divide in cases:
      \begin{itemize}
        \item If $j \le g(\sigma,i)$, then, by construction of
          $(g,B)^{w\forall}$, we have $(\sigma,j) \in B_g^2$ and by
          inductive hypothesis $(\sigma,j) \not\models \Phi_2$, which is
          a contradition.
        \item Otherwise $j>g(\sigma,i)$. In this case, by definition of
          $j$, we have that $(\sigma,g(\sigma,i)) \models \Phi_1$.  Since
          $g(\sigma,i) < |\sigma|-1$, we have $(\sigma,g(\sigma,i)) \in
          g_<(B)$ and by inductive hypothesis $(\sigma,g(\sigma,i))
          \not\models \Phi_1$, which is a contradiction.
      \end{itemize}


      Therefore, $B \pperp \ltl{\Phi U \Phi_2}$.

      It follows that $\ltl{\Phi_1 U \Phi_2}$ separates $A$ and $B$.
      Moreover, $|\ltl{\Phi_1 U \Phi_2}| = |\Phi_1| + |\Phi_2| + 1 = k$. 
  \end{description}


  $(\Leftarrow)$
  Given a formula $\Phi$ of \cosafetyltl of size $k$ such that $A \models
  \Phi$ and $B \pperp \Phi$, we build a derivation tree for $(A,B)$ of size
  $k$.

  \begin{description}
    \item[induction step: $\Phi = \ltl{\Phi_1 U \Phi_2}$.] 
      We first show that $(f,A)^{\forall} \models \Phi_1$ and $f(A) \models
      \Phi_2$ for some $f \in \FP_A$. By hypothesis, for any $a
      = (\sigma,i)$ in $A$, $(\sigma,i) \models \ltl{\Phi_1 U \Phi_2}$,
      that is there exists a $j_a \ge i$ such that $(\sigma,j_a) \models
      \Phi_2$ and $(\sigma,k) \models \Phi_1$, for all $i\le k < j_a$. We
      choose $f : A \to \N$ such that $f(a) = j_a$ for any $a \in A$. With
      this choice for $f$, for all $(\sigma',j') \in f(A)$ it holds that
      $(\sigma,j') \models \Phi_2$.  Moreover, by construction of $f$ and
      of $(f,A)^{\forall}$, it holds that $(\sigma'',j'')$ for all
      $(\sigma'',j'') \in (f,A)^{\forall}$.

      Now we prove that $g_<(B) \pperp \Phi_1$ and $(g,B)^{w\forall} \pperp
      \Phi_2$ for some $g \in \FP_B$.
      For any $(\sigma,i) \in B$, we define $g(\sigma,i)$ in this way:
      \begin{itemize}
        \item If $(\sigma,i)$ is such that $(\sigma,j) \not\models \Phi_2$
          for all $i\le j < |\sigma|$, then we define $g(\sigma,i)
          = |\sigma|-1$.
        \item If $(\sigma,i)$ is such that there exists a $j$ such that $i
          \le j < |\sigma|-1$ for which $(\sigma,j) \not\models \Phi_1$ and
          $(\sigma,k) \not\models \Phi_2$ for all $i\le k \le j$, then we
          define $g(\sigma,i) = j$.
      \end{itemize}
      Note that if $g(\sigma,i) = |\sigma|-1$, then $g_<(B)$ is the empty
      set.

      Since by hypothesis $(\sigma,i) \not\models \ltl{\Phi_1 U \Phi_2}$
      for each $(\sigma,i) \in B$, by the semantics of the \emph{until} we
      have that $(\sigma,i)$ satisfies the following condition: 
      \[\forall i\le j < |\sigma| \suchdot ((\sigma,j) \not\models \Phi_2)
      \lor \exists i\le j< |\sigma| \suchdot ((\sigma,j) \not\models \Phi_1
      \land \forall i\le k\le j \suchdot ((\sigma,k) \not\models \Phi_2))\]
      Since for $j=|\sigma_1|$ the second disjunct implies the first one,
      this is equivalent to:
      \[\forall i\le j < |\sigma| \suchdot ((\sigma,j) \not\models \Phi_2)
      \lor \exists i\le j< |\sigma|-1 \suchdot ((\sigma,j) \not\models \Phi_1
      \land \forall i\le k\le j \suchdot ((\sigma,k) \not\models \Phi_2))\]
      It follows that our choice for $g$ is indeed a function, \ie it is
      defined for all $(\sigma,i) \in B$.

      By construction of $g_<(B)$ and $(g,B)^{w\forall}$, it is easy to see
      that each $(\sigma,j) \in (g,B)^{w\forall}$ is such that $(\sigma,j)
      \not\models \Phi_2$ and that each $(\sigma,j) \in g_<(B)$ is such that
      $(\sigma,j) \not\models \Phi_1$. Therefore $g_<(B) \pperp \Phi_1$ and
      $(g,B)^{w\forall} \pperp \Phi_2$.

      Since $\Phi_1$ separates $(f,A)^{\forall}$ and $g_<(B)$ and since
      $\Phi_2$ separates $f(A)$ and $(g,B)^{w\forall}$, by inductive
      hypothesis, there are two derivation trees rooted at
      $((f,A)^{\forall},g_<(B))$ and $(f(A),(g,B)^{w\forall})$ of size
      $|\Phi_1|$ and $|\Phi_2|$, respectively. This proves that there is
      a derivation tree rooted at $(A,B)$ of size $|\Phi_1| + |\Phi_2|
      + 1$, that is $k$.
  \end{description}
\end{proof}


==> sections/subadditive.tex <==
%! root=../main.tex

\section{Sub-additive measures}
\label{sec:subadditive}

\subsection{Sub-additive proof measures for propositional logic}

In~\cite{Hella12} Hella and V\"a\"an\"anen used a
game-theoretic view of the proof system restricted to the
axiom \ruleAtomic and rules \ruleAnd and \ruleOr to show a
quadratic lower-bound for Parity on propositional formulae.
Their approach is interesting, because they tame the
combinatorics of \ruleAnd and \ruleOr by designing a
suitable function based on the Hamming distance. In this
section we abstract away from the particular function and
show that, as long as one finds a sub-additive function, the
result follows. A similar technique is used
in~\cite{Ueno13}, with interesting applications to LP.

Let $\Pi$ be the set of all pairs of set of structures
$(A,B)$ over which the proof system works. We say that a map
$\mu \colon \Pi \to \{ r \in \R : r > 0\}$ is a
\emph{sub-additive proof measure for $\Pi$} whenever it
satisfies the following properties: 
\begin{enumerate}
  \item given $A,B$ non-empty, if \ruleAtomic can be applied
  to $(A,B)$ then $\mu(A,B) \leq \min(|A|,|B|)$,
  \item for every $A_1,A_2$ such that $A = A_1 \uplus A_2$,
  we have $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$,
  \item for every $B_1,B_2$ such that $B = B_1 \uplus B_2$,
  we have $\mu(A,B) \leq \mu(A,B_1) + \mu(A,B_2)$. 
\end{enumerate}

\begin{theorem}
  \label{lemma:Hella:minimal-tree}
  Let $\mu$ be a sub-additive proof measure for $\Pi$, and
  $(A,B) \in \Pi$ with $A$ and $B$ non-empty. Every
  derivation tree for $(A,B)$ has size at least
  $\frac{\mu(A,B)^2}{|A| \cdot |B|}$.
\end{theorem}

Before proving~\Cref{lemma:Hella:minimal-tree} we need the
following result.
\begin{lemma}
  \label{lemma:Hella:and-or}
  Let $\mu$ be a sub-additive proof measure. Then,
    \begin{itemize}
      \item Let $A_1,A_2$ non-empty such that $A = A_1
      \uplus A_2$. Then, $\frac{\mu(A_1,B)^2}{|A_1|} +
      \frac{\mu(A_2,B)^2}{|A_2|} \geq
      \frac{\mu(A,B)^2}{|A|}$.
      \item Let $B_1,B_2$ non-empty such that $B = B_1
      \uplus B_2$. Then, $\frac{\mu(A,B_1)^2}{|B_1|} +
      \frac{\mu(A,B_2)^2}{|B_2|} \geq
      \frac{\mu(A,B)^2}{|B|}$.
    \end{itemize}
\end{lemma}

\begin{proof}
  We prove the first item. The proof of the second item is
  analogous. Given real numbers $x_1,x_2,w_1,w_2 > 0$,
  recall that the weighted harmonic and arithmetic means are
  defined as: 
  \begin{align}
    H \coloneqq \frac{w_1+w_2}{\frac{w_1}{x_1} + \frac{w_2}{x_2}} \tag{weighted harmonic mean}\\
    A \coloneqq \frac{w_1 \cdot x_1 + w_2 \cdot x_2}{w_1+w_2}
    \tag{weigthed arithmetic mean}
  \end{align}
  It is a well known fact that the former mean is always
  upper bounded by the latter, i.e., $H \leq A$ :
  \begin{align}
    \frac{A}{H} 
      &= \frac{w_1 \cdot x_1 + w_2 \cdot x_2}{w_1+w_2} \cdot \frac{\frac{w_1}{x_1} + \frac{w_2}{x_2}}{w_1 + w_2}\\
      &= \frac{1}{(w_1+w_2)^2} 
        \cdot (w_1 \cdot x_1 + w_2 \cdot x_2) 
        \cdot \left(\frac{w_1}{x_1} + \frac{w_2}{x_2}\right)\\
      &\geq \frac{1}{(w_1+w_2)^2}  \cdot \left(
        \sqrt{w_1 \cdot x_1} \cdot \sqrt{\frac{w_1}{x_1}} + 
        \sqrt{w_2 \cdot x_2} \cdot \sqrt{\frac{w_2}{x_2}} 
        \right)^2 
      & \text{Cauchy--Schwarz inequality}\\
      & = \frac{(w_1+w_2)^2}{(w_1+w_2)^2} = 1.
  \end{align}
  Then, the result follows using the fact that $|A| = |A_1|
  + |A_2|$ and $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$:

  \begin{align}
    \frac{\frac{\mu(A_1,B)^2}{|A_1|} +\frac{\mu(A_2,B)^2}{|A_2|}}{\mu(A,B)} 
    & 
    \geq \frac{\frac{\mu(A_1,B)^2}{|A_1|} +\frac{\mu(A_2,B)^2}{|A_2|}}{\mu(A_1,B) + \mu(A_2,B)}
    &\text{by $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$}
    \\[3pt]
    &
    \geq \frac{\mu(A_1,B) + \mu(A_2,B)}{|A_1| + |A_2|}
    &\text{from } \frac{1}{H} \geq \frac{1}{A}\\ 
    &\geq \frac{\mu(A,B)}{|A|} 
      &\text{by $|A| = |A_1| + |A_2|$ and}\\[-7pt]
    &&\text{by $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B).$}
    &\qedhere
  \end{align}
\end{proof}

\begin{proof}[Proof of~\Cref{lemma:Hella:minimal-tree}]
  We prove that for every $n \in \N$, if $(A,B)$ has a
  derivation tree of size $n$ then $n \geq
  \frac{\mu(A,B)^2}{|A| \cdot |B|}$. The proof is by
  induction on $n$.

  \begin{description}
    \item[base case: $n = 1$.] 
    Since $n = 1$, the derivation tree of $(A,B)$ must be a
    simple application of the axiom \ruleAtomic. Since $\mu$
    is a sub-additive proof measure, and $A$ and $B$ are
    non-empty, $\mu(A,B) \leq \min(|A|,|B|)$, and therefore
    $\frac{\mu(A,B)^2}{|A| \cdot |B|} \leq 1 = n$.

    \item[induction step: $n \geq 2$.] 
    Consider a derivation tree for $(A,B)$ having size $n
    \geq 2$, and observe the rule used at the root of the
    tree, i.e., the root rule. Since $n \geq 2$, the rule is
    either \ruleOr or~\ruleAnd.  
    We show that $n \geq \frac{\mu(A,B)^2}{|A| \cdot |B|}$
    for the case where the root rule is \ruleOr. The case of
    \ruleAnd is analogous.

    Let $A_1,A_2$, such that $A = A_1 \uplus A_2$, be the
    two sets considered by the root rule \ruleOr, and $n_1
    \in \N$ and $n_2 \in \N$ be the size of the derivation
    trees for $(A_1,B)$ and $(A_2,B)$. Note that we can
    assume both $A_1$ and $A_2$ to be non-empty, otherwise
    we would have $A = A_1$ or $A = A_2$ and one can modify
    the derivation tree to find a proof for $(A,B)$ of size
    $n' < n$; and obtain $n \geq \frac{\mu(A,B)^2}{|A| \cdot
    |B|}$ by induction hypothesis. So, under the assumption
    that $A_1$ and $A_2$ are non-empty, we have
    \begin{align}
      n & > n_1 + n_2 
          &\text{by definition}\\ 
        & \geq \frac{\mu(A_1,B)^2}{|A_1| \cdot |B|} + \frac{\mu(A_2,B)^2}{|A_2| \cdot |B|}
          &\text{by induction hypothesis}\\ 
        & = \frac{1}{|B|} \cdot \left( \frac{\mu(A_1,B)^2}{|A_1|} + \frac{\mu(A_2,B)^2}{|A_2|}\right)\\
        & \geq \frac{\mu(A,B)^2}{|A| \cdot |B|}
          &\text{by~\Cref{lemma:Hella:and-or}.} 
          &\qedhere
    \end{align}
  \end{description}
\end{proof}

We now show how to
instantiate~\Cref{lemma:Hella:minimal-tree} to obtain a
quadratic lower bound for the size of the formula expressing
parity. For simplicity, we consider $A,B \subseteq
\{0,1\}^k$ encoding sets of truth assignments to the
propositional symbols $\{p_0,\dots,p_{k-1}\}$. Define
$\delta_1 \colon \Pi \to \N$ to be the function:
\[
  \delta_1(A,B) \coloneqq \max(1,|\{ (a,b) \in A \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \}|).
\] 


\begin{lemma}
  \label{lemma:Hella:delta1proofmeasure}
  The function $\delta_1$ is a sub-additive proof measure.
\end{lemma}

\begin{proof}
  (1) We show the contrapositive of the first requirement of
  a sub-additive proof measure: given $A,B$ non-empty, if
  $\delta_1(A,B) > \min(|A|,|B|)$, then the axiom
  \ruleAtomic cannot be applied. Suppose $\min(|A|,|B|) =
  |A|$ (the case for $|B| = \min(|A|,|B|$) is analogous). We
  have $\delta_1(A,B) > |A|$ and so there is $a \in A$ and
  two distinct $b_1,b_2 \in B$ having Hamming distance $1$
  from $a$. Hence, for every $i \in [0,k-1]$, we have $a[i]
  = 1 \Leftrightarrow b_1[i] = 1$ or $a[i] = 1
  \Leftrightarrow b_2[i] = 1$. This implies that \ruleAtomic
  cannot be used for $p_i$ nor for $\lnot p_i$ (for all $i
  \in [0,k-1]$).

  (2) We show that $\delta_1(A,B) \leq \delta_1(A_1,B) +
  \delta_1(A_2,B)$, for all $A_1,A_2$ such that $A = A_1
  \uplus A_2$. Let, 
  \begin{align} 
    \Delta &\coloneqq \{ (a,b) \in A \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \},\\ 
    \Delta_1 &\coloneqq
    \{ (a,b) \in A_1 \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \},\\ 
    \Delta_2 &\coloneqq
    \{ (a,b) \in A_2 \times B : \text{ the Hamming distance of $a$ and $b$ is $1$} \}.
  \end{align}
  Note that, by definition, $\Delta = \Delta_1 \uplus
  \Delta_2$. If $\Delta_1$ or $\Delta_2$ are empty, then
  either $\Delta = \Delta_1$ or $\Delta = \Delta_2$, and
  thus $\delta_1(A,B) \leq \delta_1(A,B) + 1 =
  \delta_1(A_1,B) + \delta_1(A_2,B)$ follows by definition
  of $\delta_1$. Otherwise, $\Delta_1$ and $\Delta_2$ are
  non-empty and thus $\delta_1(A,B) = |\Delta| = |\Delta_1|
  + |\Delta_2| = \delta_1(A,B) + \delta_2(A,B)$, as
  required.

  (3) the proof that $\delta_1(A,B) \leq \delta_1(A,B_1) +
  \delta_1(A,B_2)$, for every $B_1,B_2$ such that $B = B_1
  \uplus B_2$, follow similarly to the previous point. 
\end{proof}


\begin{corollary}
  Let $k \geq 1$. If $\Phi$ is a propositional formula
  expressing the parity of strings $s \in \{0, 1\}^k$, then
  the size of $\Phi$ is at least $k^2$.
\end{corollary}

\begin{proof}
  Let $A \coloneqq \{ s \in \{0, 1\}^k : s \text{ has an odd
  number of $1$s} \}$ and $B \coloneqq \{0,1\}^k \setminus
  A$. Therefore, $|A| = |B| = 2^{k-1}$. For every $a \in A$,
  there are exactly $k$ different $b \in B$ having Hamming
  distance $1$ from $a$. Then, $\delta_1(A,B) = k \cdot
  2^{k-1}$ and by~\Cref{lemma:Hella:minimal-tree}
  and~\Cref{lemma:Hella:delta1proofmeasure} we conclude that
  the minimal derivation tree for $(A,B)$ as size at least
  $\frac{\delta_1(A,B)^2}{|A| \cdot |B| } = k^2$.
\end{proof}



\subsection{Sub-additive proof measures, version 2}

In fact, the definition below is a generalization of the one
in the previous section that works well for infinite models.

Let $\Pi$ be the set of all pairs of set of structures
$(A,B)$ over which the proof system works. We say that a map
$\mu \colon \Pi \to \{ r \in \R : r > 0\}$ is a
\emph{sub-additive proof measure for $\Pi$} whenever it
satisfies the following properties: 
\begin{enumerate}
  \item given $A,B$ non-empty, if \ruleAtomic can be applied
  to $(A,B)$ then $\mu(A,B) \leq 1$,
  \item for every $A_1,A_2$ such that $A = A_1 \uplus A_2$,
  we have $\mu(A,B) \leq \mu(A_1,B) + \mu(A_2,B)$,
  \item for every $B_1,B_2$ such that $B = B_1 \uplus B_2$,
  we have $\mu(A,B) \leq \mu(A,B_1) + \mu(A,B_2)$. 
\end{enumerate}

\begin{theorem}
  \label{lemma:Hella:minimal-tree-two}
  Let $\mu$ be a sub-additive proof measure for $\Pi$, and
  $(A,B) \in \Pi$ with $A$ and $B$ non-empty. Every
  derivation tree for $(A,B)$ has size at least $\mu(A,B)$.
\end{theorem}

Indeed, given a proof measure $\mu'$ defined as in the
previous section, setting $\mu(A,B) \coloneqq
\frac{\mu'(A,B)^2}{|A| \cdot |B|}$ allows us to obtain a
sub-additive proof measure w.r.t.~the above three
conditions.

For \ruleNext and \ruleFuture it seems we could add
something like: 
\begin{enumerate}
  \item[4.] $\mu(A,B) \leq \mu(A^X,B^X) + f(|A|)$ 
\end{enumerate}
where $f \colon \N \to \{ r \in \R : r \geq 0 \}$ is a fixed
monotone function. Then the theorem would become that the
minimal derivation tree of $(A,B)$ has size
$\frac{\mu(A,B)}{f(|A|)}$. So, $f$ should grow slower than
$\mu$ if we want something nice.

